Plot and Rework: Modeling Storylines for Visual Storytelling

Writing a coherent and engaging story is not easy. Creative writers use their knowledge and worldview to put disjointed elements together to form a coherent storyline, and work and rework iteratively toward perfection. Automated visual storytelling (VIST) models, however, make poor use of external knowledge and iterative generation when attempting to create stories. This paper introduces PR-VIST, a framework that represents the input image sequence as a story graph in which it finds the best path to form a storyline. PR-VIST then takes this path and learns to generate the final story via an iterative training process. This framework produces stories that are superior in terms of diversity, coherence, and humanness, per both automatic and human evaluations. An ablation study shows that both plotting and reworking contribute to the model's superiority.

==> acl2021.tex <==
@inproceedings{mitchell2018proceedings,
  title={Proceedings of the First Workshop on Storytelling},
  author={Mitchell, Margaret and Huang, Ting-Hao and Ferraro, Francis and Misra, Ishan},
  booktitle={Proceedings of the First Workshop on Storytelling},
  year={2018}
}

@article{flower1981cognitive,
  title={A cognitive process theory of writing},
  author={Flower, Linda and Hayes, John R},
  journal={College Composition and Communication},
  volume={32},
  number={4},
  pages={365--387},
  year={1981},
  publisher={JSTOR}
}

@article{dai2019transformer,
  title={Transformer-xl: Attentive language models beyond a fixed-length context},
  author={Dai, Zihang and Yang, Zhilin and Yang, Yiming and Cohen, William W and Carbonell, Jaime and Le, Quoc V and Salakhutdinov, Ruslan},
  journal={arXiv preprint arXiv:1901.02860},
  year={2019}
}

@inproceedings{vaswani2017attention,
  title={Attention is all you need},
  author={Vaswani, Ashish and Shazeer, Noam and Parmar, Niki and Uszkoreit, Jakob and Jones, Llion and Gomez, Aidan N and Kaiser, {\L}ukasz and Polosukhin, Illia},
  booktitle={Advances in Neural Information Processing Systems},
  pages={5998--6008},
  year={2017}
}
@article{devlin2018bert,
  title={Bert: Pre-training of deep bidirectional transformers for language understanding},
  author={Devlin, Jacob and Chang, Ming-Wei and Lee, Kenton and Toutanova, Kristina},
  journal={arXiv preprint arXiv:1810.04805},
  year={2018}
}
@article{liu2004conceptnet,
  title={{ConceptNet}---a practical commonsense reasoning tool-kit},
  author={Liu, Hugo and Singh, Push},
  journal={BT Technology Journal},
  volume={22},
  number={4},
  pages={211--226},
  year={2004},
  publisher={Springer}
}
@inproceedings{pengchengKnowledge2019,
  title     = {Knowledgeable {S}toryteller: A Commonsense-Driven Generative Model for Visual Storytelling},
  author    = {Yang, Pengcheng and Luo, Fuli and Chen, Peng and Li, Lei and Yin, Zhiyi and He, Xiaodong and Sun, Xu},
  booktitle = {Proceedings of the Twenty-Eighth International Joint Conference on
               Artificial Intelligence, {IJCAI-19}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},             
  pages     = {5356--5362},
  year      = {2019},
  month     = {7},
  doi       = {10.24963/ijcai.2019/744},
  url       = {https://doi.org/10.24963/ijcai.2019/744},
}
@article{hayashi2019latent,
  title={Latent relation language models},
  author={Hayashi, Hiroaki and Hu, Zecong and Xiong, Chenyan and Neubig, Graham},
  journal={arXiv preprint arXiv:1908.07690},
  year={2019}
}
@inproceedings{hsu2020knowledge,
  title={Knowledge-Enriched Visual Storytelling},
  author={Hsu, Chao-Chun and Chen, Zi-Yuan and Hsu, Chi-Yang and Li, Chih-Chia and Lin, Tzu-Yuan and Huang, Ting-Hao (Kenneth) and Ku, Lun-Wei},
  booktitle={Proceedings of Thirty-Fourth AAAI Conference on Artificial Intelligence},
  year={2020}
}
@article{chen2017multimodal,
  title={Multimodal storytelling via generative adversarial imitation learning},
  author={Chen, Zhiqian and Zhang, Xuchao and Boedihardjo, Arnold P and Dai, Jing and Lu, Chang-Tien},
  journal={arXiv preprint arXiv:1712.01455},
  year={2017}
}
@inproceedings{huang2019hierarchically,
  title={Hierarchically structured reinforcement learning for topically coherent visual story generation},
  author={Huang, Qiuyuan and Gan, Zhe and Celikyilmaz, Asli and Wu, Dapeng and Wang, Jianfeng and He, Xiaodong},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={8465--8472},
  year={2019}
}
@inproceedings{wang2018show,
  title={Show, reward and tell: Automatic generation of narrative paragraph from photo stream by adversarial training},
  author={Wang, Jing and Fu, Jianlong and Tang, Jinhui and Li, Zechao and Mei, Tao},
  booktitle={Thirty-Second AAAI Conference on Artificial Intelligence},
  year={2018}
}

@article{Jung2020HideandTellLT,
  title={Hide-and-Tell: Learning to Bridge Photo Streams for Visual Storytelling},
  author={Yunjae Jung and Dahun Kim and Sanghyun Woo and Kyungsu Kim and Sungjin Kim and In So Kweon},
  journal={ArXiv},
  year={2020},
  volume={abs/2002.00774}
}

@misc{hu2019makes,
    title={What Makes A Good Story? Designing Composite Rewards for Visual Storytelling},
    author={Junjie Hu and Yu Cheng and Zhe Gan and Jingjing Liu and Jianfeng Gao and Graham Neubig},
    year={2019},
    eprint={1909.05316},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}
@article{gonzalez2018contextualize,
  title={Contextualize, show and tell: {A} neural visual storyteller},
  author={Gonzalez-Rico, Diana and Fuentes-Pineda, Gibran},
  journal={arXiv preprint arXiv:1806.00738},
  year={2018}
}
@article{mostafazadeh2016corpus,
  title={A corpus and evaluation framework for deeper understanding of commonsense stories},
  author={Mostafazadeh, Nasrin and Chambers, Nathanael and He, Xiaodong and Parikh, Devi and Batra, Dhruv and Vanderwende, Lucy and Kohli, Pushmeet and Allen, James},
  journal={arXiv preprint arXiv:1604.01696},
  year={2016}
}

@article{kim2018glac,
  title={{GLAC Net: GLocal} {A}ttention {C}ascading {N}etworks for Multi-image Cued Story Generation},
  author={Kim, Taehyeong and Heo, Min-Oh and Son, Seonil and Park, Kyoung-Wha and Zhang, Byoung-Tak},
  journal={arXiv preprint arXiv:1805.10973},
  year={2018}
}
@article{hsu2018using,
  title={Using Inter-Sentence Diverse Beam Search to Reduce Redundancy in Visual Storytelling},
  author={Hsu, Chao-Chun and Chen, Szu-Min and Hsieh, Ming-Hsun and Ku, Lun-Wei},
  journal={arXiv preprint arXiv:1805.11867},
  year={2018}
}
@inproceedings{huang2016visual,
  title={Visual storytelling},
  author={Huang, Ting-Hao Kenneth and Ferraro, Francis and Mostafazadeh, Nasrin and Misra, Ishan and Agrawal, Aishwarya and Devlin, Jacob and Girshick, Ross and He, Xiaodong and Kohli, Pushmeet and Batra, Dhruv and others},
  booktitle={Proceedings of the 2016 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies},
  pages={1233--1239},
  year={2016}
}

@inproceedings{yang-etal-2019-enhancing-topic,
    title = "Enhancing Topic-to-Essay Generation with External Commonsense Knowledge",
    author = "Yang, Pengcheng  and
      Li, Lei  and
      Luo, Fuli  and
      Liu, Tianyu  and
      Sun, Xu",
    booktitle = "Proceedings of the 57th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2019",
    address = "Florence, Italy",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P19-1193",
    doi = "10.18653/v1/P19-1193",
    pages = "2002--2012"
}
@inproceedings{lobue-yates-2011-types,
    title = "Types of Common-Sense Knowledge Needed for Recognizing Textual Entailment",
    author = "LoBue, Peter  and
      Yates, Alexander",
    booktitle = "Proceedings of the 49th Annual Meeting of the Association for Computational Linguistics: Human Language Technologies",
    month = jun,
    year = "2011",
    address = "Portland, Oregon, USA",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P11-2057",
    pages = "329--334",
}
@inproceedings{bowman-etal-2015-large,
    title = "A large annotated corpus for learning natural language inference",
    author = "Bowman, Samuel R.  and
      Angeli, Gabor  and
      Potts, Christopher  and
      Manning, Christopher D.",
    booktitle = "Proceedings of the 2015 Conference on Empirical Methods in Natural Language Processing",
    month = sep,
    year = "2015",
    address = "Lisbon, Portugal",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D15-1075",
    doi = "10.18653/v1/D15-1075",
    pages = "632--642",
}
@article{zhang-etal-2017-ordinal,
    title = "Ordinal Common-sense Inference",
    author = "Zhang, Sheng  and
      Rudinger, Rachel  and
      Duh, Kevin  and
      Van Durme, Benjamin",
    journal = "Transactions of the Association for Computational Linguistics",
    volume = "5",
    year = "2017",
    url = "https://www.aclweb.org/anthology/Q17-1027",
    doi = "10.1162/tacl_a_00068",
    pages = "379--395",
}
@inproceedings{ijcai2018-643,
  title     = {Commonsense Knowledge Aware Conversation Generation with Graph Attention},
  author    = {Hao Zhou and Tom Young and Minlie Huang and Haizhou Zhao and Jingfang Xu and Xiaoyan Zhu},
  booktitle = {Proceedings of the Twenty-Seventh International Joint Conference on
               Artificial Intelligence, {IJCAI-18}},
  publisher = {International Joint Conferences on Artificial Intelligence Organization},             
  pages     = {4623--4629},
  year      = {2018},
  month     = {7},
  doi       = {10.24963/ijcai.2018/643},
  url       = {https://doi.org/10.24963/ijcai.2018/643},
}
@article{DBLP:journals/corr/abs-1808-10113,
  author    = {Jian Guan and
               Yansen Wang and
               Minlie Huang},
  title     = {Story Ending Generation with Incremental Encoding and Commonsense
               Knowledge},
  journal   = {CoRR},
  volume    = {abs/1808.10113},
  year      = {2018},
  url       = {http://arxiv.org/abs/1808.10113},
  archivePrefix = {arXiv},
  eprint    = {1808.10113},
  timestamp = {Mon, 03 Sep 2018 13:36:40 +0200},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1808-10113},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@inproceedings{kikuchi-etal-2016-controlling,
    title = "Controlling Output Length in Neural Encoder-Decoders",
    author = "Kikuchi, Yuta  and
      Neubig, Graham  and
      Sasano, Ryohei  and
      Takamura, Hiroya  and
      Okumura, Manabu",
    booktitle = "Proceedings of the 2016 Conference on Empirical Methods in Natural Language Processing",
    month = nov,
    year = "2016",
    address = "Austin, Texas",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/D16-1140",
    doi = "10.18653/v1/D16-1140",
    pages = "1328--1338",
}
@inproceedings{takase-okazaki-2019-positional,
    title = "Positional Encoding to Control Output Sequence Length",
    author = "Takase, Sho  and
      Okazaki, Naoaki",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/N19-1401",
    doi = "10.18653/v1/N19-1401",
    pages = "3999--4004",
    
}
@article{Alexander2018Semstyle,
  author    = {Alexander Patrick Mathews and
               Lexing Xie and
               Xuming He},
  title     = {SemStyle: Learning to Generate Stylised Image Captions using Unaligned Text},
  journal   = {CoRR},
  volume    = {abs/1805.07030},
  year      = {2018}
}
@article{swayamdipta17open,
  title={{Frame-Semantic Parsing with Softmax-Margin Segmental RNNs and a Syntactic Scaffold}},
  author={Swabha Swayamdipta and Sam Thomson and Chris Dyer and Noah A. Smith},
  journal={arXiv preprint arXiv:1706.09528},
  year={2017}
}
@inproceedings{baker1998berkeley,
  title={{The Berkeley FrameNet Project}},
  author={Baker, Collin F and Fillmore, Charles J and Lowe, John B},
  booktitle={Proceedings of the 17th International Conference on Computational Linguistics-Volume 1},
  pages={86--90},
  year={1998},
  organization={Association for Computational Linguistics}
}

@inproceedings{ren2015faster,
  title={{Faster R-CNN}: Towards real-time object detection with region proposal networks},
  author={Ren, Shaoqing and He, Kaiming and Girshick, Ross and Sun, Jian},
  booktitle={Advances in Neural Information Processing Systems},
  pages={91--99},
  year={2015}
}
@inproceedings{anderson2018bottom,
  title={Bottom-up and top-down attention for image captioning and visual question answering},
  author={Anderson, Peter and He, Xiaodong and Buehler, Chris and Teney, Damien and Johnson, Mark and Gould, Stephen and Zhang, Lei},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={6077--6086},
  year={2018}
}

@article{chung2014empirical,
  title={Empirical evaluation of gated recurrent neural networks on sequence modeling},
  author={Chung, Junyoung and Gulcehre, Caglar and Cho, KyungHyun and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1412.3555},
  year={2014}
}


@article{DBLP:journals/corr/abs-1804-09160,
  author    = {Xin Wang and
               Wenhu Chen and
               Yuan{-}Fang Wang and
               William Yang Wang},
  title     = {No Metrics Are Perfect: Adversarial Reward Learning for Visual Storytelling},
  journal   = {CoRR},
  volume    = {abs/1804.09160},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.09160},
  archivePrefix = {arXiv},
  eprint    = {1804.09160},
  timestamp = {Tue, 26 Nov 2019 08:07:50 +0100},
  biburl    = {https://dblp.org/rec/bib/journals/corr/abs-1804-09160},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
%UHop
@misc{chen2019uhop,
    title={{UHop}: An Unrestricted-Hop Relation Extraction Framework for Knowledge-Based Question Answering},
    author={Zi-Yuan Chen and Chih-Hung Chang and Yi-Pei Chen and Jijnasa Nayak and Lun-Wei Ku},
    year={2019},
    eprint={1904.01246},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}
@article{Yu_2018,
   title={Knowledge Base Relation Detection via Multi-View Matching},
   ISBN={9783030000639},
   ISSN={1865-0937},
   url={http://dx.doi.org/10.1007/978-3-030-00063-9_27},
   DOI={10.1007/978-3-030-00063-9_27},
   journal={New Trends in Databases and Information Systems},
   publisher={Springer International Publishing},
   author={Yu, Yang and Hasan, Kazi Saidul and Yu, Mo and Zhang, Wei and Wang, Zhiguo},
   year={2018},
   pages={286–294}
}


@inproceedings{hu20aaai,
    title = {What Makes A Good Story? {D}esigning Composite Rewards for Visual Storytelling},
    author = {Junjie Hu and Yu Cheng and Zhe Gan and Jingjing Liu and Jianfeng Gao and Graham Neubig},
    booktitle = {Thirty-Fourth AAAI Conference on Artificial Intelligence (AAAI)},
    address = {New York, USA},
    month = {February},
    url = {https://arxiv.org/abs/1909.05316},
    year = {2020}
}
@inproceedings{wang2019hierarchical,
  title={Hierarchical photo-scene encoder for album storytelling},
  author={Wang, Bairui and Ma, Lin and Zhang, Wei and Jiang, Wenhao and Zhang, Feng},
  booktitle={Proceedings of the AAAI Conference on Artificial Intelligence},
  volume={33},
  pages={8909--8916},
  year={2019}
}
@inproceedings{Wang2020StorytellingFA,
  title={Storytelling from an Image Stream Using Scene Graphs},
  author={Ruize Wang and Zhongyu Wei and Piji Li and Qi Zhang and Xuanjing Huang},
  booktitle={AAAI 2020},
  year={2020}
}
@inproceedings{yang2019auto,
  title={Auto-encoding scene graphs for image captioning},
  author={Yang, Xu and Tang, Kaihua and Zhang, Hanwang and Cai, Jianfei},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition},
  pages={10685--10694},
  year={2019}
}
@article{DBLP:journals/corr/abs-1803-01271,
  author    = {Shaojie Bai and
               J. Zico Kolter and
               Vladlen Koltun},
  title     = {An Empirical Evaluation of Generic Convolutional and Recurrent Networks
               for Sequence Modeling},
  journal   = {CoRR},
  volume    = {abs/1803.01271},
  year      = {2018},
  url       = {http://arxiv.org/abs/1803.01271},
  archivePrefix = {arXiv},
  eprint    = {1803.01271},
  timestamp = {Mon, 13 Aug 2018 16:47:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1803-01271.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1804-01622,
  author    = {Justin Johnson and
               Agrim Gupta and
               Li Fei{-}Fei},
  title     = {Image Generation from Scene Graphs},
  journal   = {CoRR},
  volume    = {abs/1804.01622},
  year      = {2018},
  url       = {http://arxiv.org/abs/1804.01622},
  archivePrefix = {arXiv},
  eprint    = {1804.01622},
  timestamp = {Sat, 19 Oct 2019 16:30:04 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1804-01622.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
%evaluation metrics
@article{DBLP:journals/corr/abs-1904-09675,
  author    = {Tianyi Zhang and
               Varsha Kishore and
               Felix Wu and
               Kilian Q. Weinberger and
               Yoav Artzi},
  title     = {BERTScore: Evaluating Text Generation with {BERT}},
  journal   = {CoRR},
  volume    = {abs/1904.09675},
  year      = {2019},
  url       = {http://arxiv.org/abs/1904.09675},
  archivePrefix = {arXiv},
  eprint    = {1904.09675},
  timestamp = {Wed, 03 Jun 2020 10:08:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1904-09675.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@misc{sellam2020bleurt,
    title={{BLEURT}: Learning Robust Metrics for Text Generation},
    author={Thibault Sellam and Dipanjan Das and Ankur P. Parikh},
    year={2020},
    eprint={2004.04696},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@article{Lexical,
 URL = {https://doi.org/10.3758/BRM.42.2.381},
 author = {McCarthy and Jarvis, S.},
 pages = {381–392},
 title = {{MTLD, vocd-D, and HD-D}: A validation study of sophisticated approaches to lexical diversity assessment},
 journal = {Behavior Research Methods},
 year = {2010}
}



@article{10.2307/1473169,
 ISSN = {15554023},
 URL = {http://www.jstor.org/stable/1473169},
 author = {Edgar Dale and Jeanne S. Chall},
 journal = {Educational Research Bulletin},
 number = {1},
 pages = {11--28},
 publisher = {Taylor & Francis, Ltd.},
 title = {A Formula for Predicting Readability},
 volume = {27},
 year = {1948}
}


@article{DBLP:journals/corr/abs-1811-05701,
  author    = {Lili Yao and
               Nanyun Peng and
               Ralph M. Weischedel and
               Kevin Knight and
               Dongyan Zhao and
               Rui Yan},
  title     = {Plan-And-Write: Towards Better Automatic Storytelling},
  journal   = {CoRR},
  volume    = {abs/1811.05701},
  year      = {2018},
  url       = {http://arxiv.org/abs/1811.05701},
  archivePrefix = {arXiv},
  eprint    = {1811.05701},
  timestamp = {Sat, 31 Aug 2019 16:23:05 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1811-05701.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1902-01109,
  author    = {Angela Fan and
               Mike Lewis and
               Yann N. Dauphin},
  title     = {Strategies for Structuring Story Generation},
  journal   = {CoRR},
  volume    = {abs/1902.01109},
  year      = {2019},
  url       = {http://arxiv.org/abs/1902.01109},
  archivePrefix = {arXiv},
  eprint    = {1902.01109},
  timestamp = {Mon, 22 Jul 2019 13:15:46 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1902-01109.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/abs-1906-01764,
  author    = {Ting{-}Yao Hsu and
               Chieh{-}Yang Huang and
               Yen{-}Chia Hsu and
               Ting{-}Hao Kenneth Huang},
  title     = {Visual Story Post-Editing},
  journal   = {CoRR},
  volume    = {abs/1906.01764},
  year      = {2019},
  url       = {http://arxiv.org/abs/1906.01764},
  archivePrefix = {arXiv},
  eprint    = {1906.01764},
  timestamp = {Thu, 13 Jun 2019 13:36:00 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1906-01764.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@inproceedings{10.1145/3323873.3325050,
author = {Li, Nanxing and Liu, Bei and Han, Zhizhong and Liu, Yu-Shen and Fu, Jianlong},
title = {Emotion Reinforced Visual Storytelling},
year = {2019},
isbn = {9781450367653},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3323873.3325050},
doi = {10.1145/3323873.3325050},
booktitle = {Proceedings of the 2019 on International Conference on Multimedia Retrieval},
pages = {297–305},
numpages = {9},
keywords = {storytelling, emotion, reinforcement learning, multi-modal},
location = {Ottawa ON, Canada},
series = {ICMR '19}
}

%dataset
@article{Krishna_2017,
   title={Visual {G}enome: Connecting Language and Vision Using Crowdsourced Dense Image Annotations},
   volume={123},
   ISSN={1573-1405},
   url={http://dx.doi.org/10.1007/s11263-016-0981-7},
   DOI={10.1007/s11263-016-0981-7},
   number={1},
   journal={International Journal of Computer Vision},
   publisher={Springer Science and Business Media LLC},
   author={Krishna, Ranjay and Zhu, Yuke and Groth, Oliver and Johnson, Justin and Hata, Kenji and Kravitz, Joshua and Chen, Stephanie and Kalantidis, Yannis and Li, Li-Jia and Shamma, David A. and et al.},
   year={2017},
   month={Feb},
   pages={32–73}
}
@inproceedings{pennington2014glove,
  author = {Jeffrey Pennington and Richard Socher and Christopher D. Manning},
  booktitle = {Empirical Methods in Natural Language Processing (EMNLP)},
  title = {{GloVe}: Global Vectors for Word Representation},
  year = {2014},
  pages = {1532--1543},
  url = {http://www.aclweb.org/anthology/D14-1162},
}

% RL
@article{10.1007/BF00992696,
author = {Williams, Ronald J.},
title = {Simple Statistical Gradient-Following Algorithms for Connectionist Reinforcement Learning},
year = {1992},
issue_date = {May 1992},
publisher = {Kluwer Academic Publishers},
address = {USA},
volume = {8},
number = {3–4},
issn = {0885-6125},
url = {https://doi.org/10.1007/BF00992696},
doi = {10.1007/BF00992696},
journal = {Mach. Learn.},
month = may,
pages = {229–256},
numpages = {28},
keywords = {gradient descent, connectionist networks, Reinforcement learning, mathematical analysis}
}
%image caption  task
@article{Fang_2015,
   title={From captions to visual concepts and back},
   ISBN={9781467369640},
   url={http://dx.doi.org/10.1109/CVPR.2015.7298754},
   DOI={10.1109/cvpr.2015.7298754},
   journal={2015 IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
   publisher={IEEE},
   author={Fang, Hao and Gupta, Saurabh and Iandola, Forrest and Srivastava, Rupesh K. and Deng, Li and Dollar, Piotr and Gao, Jianfeng and He, Xiaodong and Mitchell, Margaret and Platt, John C. and et al.},
   year={2015},
   month={Jun}
}
%story plotting citation
@article{Ammanabrolu_2020,
   title={Story Realization: Expanding Plot Events into Sentences},
   volume={34},
   ISSN={2159-5399},
   url={http://dx.doi.org/10.1609/aaai.v34i05.6232},
   DOI={10.1609/aaai.v34i05.6232},
   number={05},
   journal={Proceedings of the AAAI Conference on Artificial Intelligence},
   publisher={Association for the Advancement of Artificial Intelligence (AAAI)},
   author={Ammanabrolu, Prithviraj and Tien, Ethan and Cheung, Wesley and Luo, Zhaochen and Ma, William and Martin, Lara J. and Riedl, Mark O.},
   year={2020},
   month={Apr},
   pages={7375–7382}
}
@article{jamesscottbell_plot,
   title={Plot \& Structure: Techniques and Exercises for Crafting a Plot That Grips Readers from Start to Finish},
   publisher={Writer’s Digest Books},
   author={James Scott Bell},
   year={2004},
}

@article{Yao_2019,
   title={Plan-and-Write: Towards Better Automatic Storytelling},
   volume={33},
   ISSN={2159-5399},
   url={http://dx.doi.org/10.1609/aaai.v33i01.33017378},
   DOI={10.1609/aaai.v33i01.33017378},
   journal={Proceedings of the AAAI Conference on Artificial Intelligence},
   publisher={Association for the Advancement of Artificial Intelligence (AAAI)},
   author={Yao, Lili and Peng, Nanyun and Weischedel, Ralph and Knight, Kevin and Zhao, Dongyan and Yan, Rui},
   year={2019},
   month={Jul},
   pages={7378–7385}
}
@article{stephenking_edit,
   title={On Writing: A Memoir of the Craft},
   publisher={New York: Scribner},
   author={Stephen King},
   year={2000},
}
@article{marktwain_edit,
   title={The Adventures of Tom Sawyer},
   publisher={American Publishing Company},
   author={Mark Twain},
   year={1876},
}
@inproceedings{modi-parde-2019-steep,
    title = "The Steep Road to Happily Ever After: An Analysis of Current Visual Storytelling Models",
    author = "Modi, Yatri  and
      Parde, Natalie",
    booktitle = "Proceedings of the Second Workshop on Shortcomings in Vision and Language",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/W19-1805",
    doi = "10.18653/v1/W19-1805",
    pages = "47--57",
}
@article{DBLP:journals/corr/LiGBGD15,
  author    = {Jiwei Li and
               Michel Galley and
               Chris Brockett and
               Jianfeng Gao and
               Bill Dolan},
  title     = {A Diversity-Promoting Objective Function for Neural Conversation Models},
  journal   = {CoRR},
  volume    = {abs/1510.03055},
  year      = {2015},
  url       = {http://arxiv.org/abs/1510.03055},
  archivePrefix = {arXiv},
  eprint    = {1510.03055},
  timestamp = {Mon, 13 Aug 2018 16:46:10 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/LiGBGD15.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@article{DBLP:journals/corr/ShaoGBGSK17,
  author    = {Louis Shao and
               Stephan Gouws and
               Denny Britz and
               Anna Goldie and
               Brian Strope and
               Ray Kurzweil},
  title     = {Generating Long and Diverse Responses with Neural Conversation Models},
  journal   = {CoRR},
  volume    = {abs/1701.03185},
  year      = {2017},
  url       = {http://arxiv.org/abs/1701.03185},
  archivePrefix = {arXiv},
  eprint    = {1701.03185},
  timestamp = {Mon, 13 Aug 2018 16:48:39 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/ShaoGBGSK17.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}
@misc{bahdanau2014neural,
  author = {Bahdanau, Dzmitry and Cho, Kyunghyun and Bengio, Yoshua},
  biburl = {https://www.bibsonomy.org/bibtex/2713375898fd7d2477f6ab6dc3dd66c2c/jan.hofmann1},
  description = {[1409.0473] Neural Machine Translation by Jointly Learning to Align and Translate},
  interhash = {bb2ca011eeafccb0bd2505c9476dcd10},
  intrahash = {713375898fd7d2477f6ab6dc3dd66c2c},
  keywords = {thema:pyramid_scene_parsing},
  note = {cite arxiv:1409.0473 (Accepted at ICLR 2015 as an oral presentation)},
  timestamp = {2020-06-07T20:24:58.000+0200},
  title = {Neural Machine Translation by Jointly Learning to Align and Translate},
  url = {http://arxiv.org/abs/1409.0473},
  year = 2014
}
@article{DBLP:journals/corr/abs-1709-08878,
  author    = {Kelvin Guu and
               Tatsunori B. Hashimoto and
               Yonatan Oren and
               Percy Liang},
  title     = {Generating Sentences by Editing Prototypes},
  journal   = {CoRR},
  volume    = {abs/1709.08878},
  year      = {2017},
  url       = {http://arxiv.org/abs/1709.08878},
  archivePrefix = {arXiv},
  eprint    = {1709.08878},
  timestamp = {Mon, 13 Aug 2018 16:46:37 +0200},
  biburl    = {https://dblp.org/rec/journals/corr/abs-1709-08878.bib},
  bibsource = {dblp computer science bibliography, https://dblp.org}
}

@article{10.5555/2566972.2566993,
author = {Hodosh, Micah and Young, Peter and Hockenmaier, Julia},
title = {Framing Image Description as a Ranking Task: Data, Models and Evaluation Metrics},
year = {2013},
issue_date = {May 2013},
publisher = {AI Access Foundation},
address = {El Segundo, CA, USA},
volume = {47},
number = {1},
issn = {1076-9757},
journal = {J. Artif. Int. Res.},
month = may,
pages = {853–899},
numpages = {47}
}
@inproceedings{kuznetsova-etal-2013-generalizing,
    title = "Generalizing Image Captions for Image-Text Parallel Corpus",
    author = "Kuznetsova, Polina  and
      Ordonez, Vicente  and
      Berg, Alexander  and
      Berg, Tamara  and
      Choi, Yejin",
    booktitle = "Proceedings of the 51st Annual Meeting of the Association for Computational Linguistics (Volume 2: Short Papers)",
    month = aug,
    year = "2013",
    address = "Sofia, Bulgaria",
    publisher = "Association for Computational Linguistics",
    url = "https://www.aclweb.org/anthology/P13-2138",
    pages = "790--796",
}
%optimizer
@misc{kingma2014adam,
    title={Adam: A Method for Stochastic Optimization},
    author={Diederik P. Kingma and Jimmy Ba},
    year={2014},
    eprint={1412.6980},
    archivePrefix={arXiv},
    primaryClass={cs.LG}
}
@misc{wang2019consistent,
    title={Keep it Consistent: Topic-Aware Storytelling from an Image Stream via Iterative Multi-agent Communication},
    author={Ruize Wang and Zhongyu Wei and Piji Li and Haijun Shan and Ji Zhang and Qi Zhang and Xuanjing Huang},
    year={2019},
    eprint={1911.04192},
    archivePrefix={arXiv},
    primaryClass={cs.CL}
}

@article{Li_2020,
   title={Topic Adaptation and Prototype Encoding for Few-Shot Visual Storytelling},
   ISBN={9781450379885},
   url={http://dx.doi.org/10.1145/3394171.3413886},
   DOI={10.1145/3394171.3413886},
   journal={Proceedings of the 28th ACM International Conference on Multimedia},
   publisher={ACM},
   author={Li, Jiacheng and Tang, Siliang and Li, Juncheng and Xiao, Jun and Wu, Fei and Pu, Shiliang and Zhuang, Yueting},
   year={2020},
   month={Oct}
}
@InProceedings{Liu_2019_ICCV,
author = {Liu, Lixin and Tang, Jiajun and Wan, Xiaojun and Guo, Zongming},
title = {Generating Diverse and Descriptive Image Captions Using Visual Paraphrases},
booktitle = {Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
month = {October},
year = {2019}
}

@inproceedings{dai2017towards,
  title={Towards diverse and natural image descriptions via a conditional {GAN}},
  author={Dai, Bo and Fidler, Sanja and Urtasun, Raquel and Lin, Dahua},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision},
  pages={2970--2979},
  year={2017}
}
@article{cho2014learning,
  title={Learning phrase representations using {RNN} encoder-decoder for statistical machine translation},
  author={Cho, Kyunghyun and Van Merri{\"e}nboer, Bart and Gulcehre, Caglar and Bahdanau, Dzmitry and Bougares, Fethi and Schwenk, Holger and Bengio, Yoshua},
  journal={arXiv preprint arXiv:1406.1078},
  year={2014}
}


==> origin/ablation-orig.tex <==
\section{Ablation Study}
\input{tables/ablation_test}
There are three factors contribute to {\system}'s out-performance: story
elements, knowledge graphs, and plot-rework. 
To evaluate the effectiveness of each factor in our framework, we conduct three
ablation studies by using human evaluations. The evaluation results are shown
in Table~\ref{tb:ablation_test}. All three experiments are same as qualitative
analysis, and each experiment ranks {\system} and two ablation settings whose
certain components are removed.

\paragraph{Story Elements}
{\system} is compared to two ablation models, each of them only uses $objects$
or $terms$ for storyline predictor to plot storylines. 
\paragraph{Knowledge Graphs}
{\system} is compared to two ablation models, each of them only uses
\(\mathcal{G}_{\mathit{vist}}\) or \(\mathcal{G}_{\mathit{vg}}\) for storyline
predictor to plot storylines.  
\paragraph{Plot and Rework}
%evaluated two of the settings of {\system}: one without plotting and one without reworking. 
{\system} is compared to two ablation models: without-reworking and
without-plotting-reworking. Without-reworking means the removal of
discriminator, that is, story generator uses Equation \ref{story_equation} for
all epochs. For without-plotting-reworking, we further remove the storyline
predictor: no frames are included; $terms$ are used directly as story
generator's input.
%In the table,
%{\system} differs notably in terms of rank and standard deviation from 
%{\system} w/o PR. This indicates that the influence of each stage on
%stability and story quality increases gradually. 
%Given a notable different between \system and \system w/o RE, we story plotting dominates the stability and the quality of our story.
%\subsection{Ablation Study Analysis}

Table~\ref{tb:ablation_test} shows {\system} outperforms all the ablation
models. Furthermore, the first and second experiments also show MTurkers prefer
story-like storyline than image-like storyline. That is $terms$ and
\(\mathcal{G}_{\mathit{vist}}\) are better than $objects$ and
\(\mathcal{G}_{\mathit{vg}}\). For third experiment, there's a steady
improvement from without-plotting-reworking to {\system}, showing proposed
method's effectiveness. An example is demonstrated in Figure~\ref{fig:without}.
The model cannot manage the abundant story elements without the guidance of
story plotting.
%After story plotting, the storyline prediction model organizes and
%associates the story elements, and thus generates coherent sentences. 
Comparing {\system} with {\system} w/o R, reworking revises and
enlivens (e.g., ``[organization] in [location]''). 
% \yun{For ablation study, did you run another human eval similarly but with three models? So judges rank them 1 to 3?}
%\input{tables/ablation}

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth ]{figures/without.pdf}
	 \caption{Snippet of stories generated by proposed method and two
	 configurations:
	 without reworking (w/o R) and without plotting-reworking (w/o PR). Nouns
	 and verb frames are denoted as words in blue and red. Reworking's edits on
	 stories are highlighted by wavy underlines.} 
    \label{fig:without}
\end{figure}


==> origin/abstract-orig.tex <==
\begin{abstract}

Writing a coherent and engaging story is hard.
Creative writers use their knowledge and worldview to put disjointed elements together to form a coherent storyline, and work and rework iteratively toward perfection.
Automated visual storytelling (VIST) models, however, underused external knowledge and iterative generation to create vivid stories.
This paper introduces \textit{\textbf{\system}}, a framework that 
represents the input image sequence as one ``Story Graph'' 
%by linking all the images' elements together using external knowledge,
and finds the best path in the graph to form a storyline.
\system then takes the found path and learns to generate the final story in through iterative process training process.
This framework produces stories that advance in diversity, coherence, and humanness, per both automatic and human evaluations.
The ablation study shows that both plotting and reworking contribute to the model's superiority.
%We believe 
%This work shows plausibility of drawing insights from human writers' cognitive processes or
%behaviors to improve story generation.

%can also encourage others to seek for inspirations from human writers' behaviors 


%keep communities in the center of every AI system design stage.

%Experimental results using both automatic and human evaluations demonstrate 
%{\system}'s advantages in diversity, coherence, and
%humanness. 

%to connect all the elements in the input image sequence to form a graph




\end{abstract}

%------------- dead kitten ----------

\begin{comment}

%~\ethan{Boaz says we're missing ``re'' in the title}
Visual storytelling (VIST): generates a story given five images, marks an important keystone in vision-to-language. %To systematize story writing,
Professional authors apply two story-writing skills 
to structure their writing process: \textit{story-plotting} and \textit{story-reworking}. Story-plotting organizes disjointed elements and knowledge into a storyline, and story-reworking improves the story-writing skill. 
%However, recent end-to-end frameworks directly input images to generate a story, 
However, recent studies fail utilize real-world knowledge for storyline plotting, and the generated stories remain machine-like. 
% automatically evaluate and refine stories aligning with human judgement.%disabling the frameworks from embedding story plotting and story editing process. %manipulating the visual elements or generated stories.
%\lwku{we did not focus on manipulating in this paper right?}
%\ethan{fixed}
%However, these frameworks aren't capable of diversify and organize visual elements or flex and refine the generated stories. 
%While recent frameworks only observe and write a story,
%, this paper adopts two story writing concepts: \textit{story plotting} and \textit{editing}. That is, story plotting organizes a sequence of fragmentary events before writing a story, and story editing refines the writing style after generating a story. 
%{\system} consists three stages, which it \textit{observes, plans, write-edits} the story.
%Imitating writer's behavior, {\system} %observes, 
%plans, write-edits the stories. 
%To this end,
Inspired by the human writing process, we propose \textbf{\system}, a novel
story-\textbf{p}lotting and -\textbf{re}working framework to write
coherent human-like stories. 
% consists of a story plotting stage and a story re-editing stage. 
%the aforementioned concepts.  %{\system}
First, the system utilizes the knowledge graphs and extracts story elements. In the story-plotting stage, we transform each five images into a story graph.   
%First,  
%Along with these concepts, 
%from a multi-aspect knowledge graph, which brings in vision and story intuitions. %to construct a \ethan{story-graph}, customized for each image sequences.
%After creating a \ethan{story-graph}, 
%Second, 
A model pathfinds a storyline in the graph, outlining the story arc of the images. %strategically %before story generation. 
%Lastly, 
%The story generation model receives and handles various storyline lengths to generates a preliminary story. 
%After generating a preliminary story from a storyline,
%Then, 
In the reworking stage, the story generator  generates the story from the storyline; a story evaluator also optimizes the model toward human preference.
%A discriminator 
%with reward function 
%that mimics human preference to rate the generated story. The generation model then refine the story accordingly to the score. 
%As a result, 
% Finally,
% we argue our stories tackles four %human-preferred
% unique
% aspects which the framework \textit{diversifies} and \textit{organizes} the visual elements, as well as, \textit{elasticises} and \textit{refines} the stories. %diversity, organization, elasticity, and refinement.
% Experimental results with automatic and human evaluations demonstrate that the proposed framework, plotting and editing, benefits visual story quality.
We argue the proposed framework improves visual stories by organizing
the story elements and reworking the stories.
Experimental results using both automatic and human evaluations demonstrate 
{\system}'s advantages in diversity, coherence, and
humanness. 
%\ethan{fixed, go fix e.g. remove e.q., and reasoning after first sentence}


% -1st advantage: increase stories' diversity

% -2nd advantage: coherent events that best describe 5 images

% -3rd advantage: bring in the view of human judgement 

%\ethan{
%Diversify: Diversity matrix.

%Organize: With and without planning ablation study.

%Elasticise: Calculate our story length.

%Refine: With and without discriminator ablation study.

%Should I explicitly write four aspects? or various aspects?

%editing or refining?}



% Visual Storytelling is characterized as a vision-to-language task, which the goal is to write a story from a sequence of images. 
% %Recent works implemented sophisticate end-to-end vision-to-language approaches to enhance story's relevance. 
% %Other works applied knowledge graph and scene graph that learned the cross-image relations and increased the story cohesion. 
% However, the most of studies didn't consider the storyline in storytelling, hence those works are hard to narrate a story with a dependent theme or the emphasis on causality.
% Given a sequence of images, this paper emphasized on plotting a storyline for object and action entities.  
% We proposed Story-Plotting Visual Storytelling, a three-stage knowledge-based visual storytelling framework that is able to construct story lines and generate cohesive stories.
% The framework consists knowledge graph based relation prediction model and story generation model.
% In the first stage, the frameworks transforms the images into object-action graphs. 
% Then, the relation prediction model prosecutes an multi-hop relation prediction for story-plotting. 
% In the last stage, the \yun{hierarchical} Transformer generates stories based on the predicted storyline. 
% \yun{ When generating stories, we also proposed a reinforcement learning framework, with reward function designed to select human-like stories, to adjust generated stories.} 
% The human evaluation shows the story quality is improved after implementing the proposed framework. 
% \yun{Both automatic and human evaluations show that...(if automatic metric improves)}



\end{comment}


==> origin/auto-eval-result-orig.tex <==

%For the readers reference, 
Table~\ref{tb:auto_new} shows the automatic evaluation results.
The proposed method outperforms all the baselines in the state-of-the-art
BERT-based metric and lexical diversity metrics.

While n-gram-based automatic metrics are known to correlate poorly with human
judgments for the VIST task, it is still noteworthy that the proposed method
results in significantly lower BLEU-4 scores.
{\system} was designed to utilize large scope of real-world knowledge, that is,
the story elements and knowledge graph relations.
We suspect that the use of rich vocabularies and knowledge enrich the story
content and increase lexical diversity, but also lower the performance in
n-gram matching.
%, even when BLEURT computes high semantic similarity. 
To evaluate ability in utilizing intra-image entities, we calculate the ratio
of the generated stories that use story elements from two (or above) images,
which {\system} lands 57.3\
%. %It indicates our system can manipulate the information across images.
%Moreover, the storyline prediction can employ explicit story element to enhance stories' detail and increase diversity.
In addition, in text generation, lengthier text usually has low diversity.
However, our model generates longer stories (5.96 sentences on average) than
baseline models (5 sentences on average) with a higher diversity score.


\input{tables/new_auto}

%------------------- dead kitten -----------------

\begin{comment}


the performance on n-gram-based metrics, a BERT-based metric, and diversity metrics.


n-gram-based automatic metrics such as BLEU and METEOR are commonly used in text generation evaluation. 
However, a large set of prior VIST work have shown that the classic automatic evaluation scores, correlate poorly with human judgments



% Some works \cite{wang2018show, modi-parde-2019-steep} have confirm that n-gram based automatic evaluation metrics(i.e., METROR, ROUGE-L, CIDEr, and BLEU) do not correlate well with human evaluations. 
% in language generation, but here we still adopt these metrics for reference. \yun{delete}
%Indeed, the values show a strong disagreement between two type of metrics. 
%Though our method obtains lower scores on n-gram based metrics, the higher score on the BERT-based metric can be inferred that our model %do not overfit on VIST dataset and can get higher agreement from human. ~\ethan{why does it indicate not overfit, or higher agreement from human?}
Despite our method's lower scores in n-gram based metrics, it scores significant higher in the state-of-the-art BERT-based metric and lexical diversity metric. 
The contrary results between n-gram based metrics and the others are caused by difference in our framework design. 
%{\system} was designed to tell the stories similar to the ground-truth, yet elaborate its stories using different vocabulary. 
{\system} was designed to utilize large scope of real-world knowledge, that is, the story elements and knowledge graph relations. 
The usage of rare vocabularies in real-world knowledge can enrich the story content and increase lexical diversity, but it can also lower the performance in n-gram matching, even when BLEURT computes high semantic similarity. 
In contrary, the baseline models: AREL and GLAC, generate simple and monotonous stories. Simple stories performed well in n-gram based metrics, but failed to mention details in the images. As a result, they perform poorly in BLEURT and diversity metrics. 
Notably, the advantage of {\system} over KG-Story indicates our model has an upper hand in story planning. 
Utilizing multiple knowledge graphs and story elements allows diverse knowledge which benefits overall story quality.
%This can imply the generated stories contain high vocabulary diversity, but the story
%semantics remain related to the golden stories in VIST. Thus, the 

%\yun{Note partial reason for the lower automatic measures of the proposed model compared with baseline might attributed to the fact that the proposed model doesn't necessarily generate 5-sentence long as the reference story.}

%The diversity and repetition metrics in Table~\ref{tb:auto_diverse} show that two
%end-to-end models (AREL and GLAC) fail to generate diverse and concise stories
%compared with graph-based methods (KG-Story and {\system}), which utilize
%external sources.


% \input{tables/automatic_gram}
% \input{tables/automatic_diverse}

\end{comment}


==> origin/conclusion-orig.tex <==
\section{Conclusion}
We propose a novel story plotting and reworking framework to mimic the human
story-writing process. To the best of our knowledge, no research has integrated
knowledge graph and story plotting to utilize visual elements in VIST. Also
novel is our approximation of human-preferred stories by reusing and
aggregating story generation using the results of human-annotated story ranking
evaluations, e.g., human evaluation results from MTurk.
We also propose a novel questionnaire embedded in the comparative study to
collect detailed, meaningful human-annotated data from MTurk.
%innovative approach to utilize visual element by story plotting and reuses the story ranking evaluation result. 
Experiments attest {\system}'s strong performance in diversity, coherence, and
humanness.


==> origin/discussion-orig.tex <==
\section{Discussion}

To understand the potential areas of improvement, in the human ranking
evaluation, we ask crowd workers to select the aspect(s) (out of six) they
dislike about the worst story.
24.6\% of the dislike votes are ``grounding.''
Namely, the lower-ranked stories are often not visually grounded.
We look into the outputs and found that the Faster-RCNN in Stage 1 sometimes
predicts objects that are inaccurate but semantically related to the context.
Figure~\ref{fig:error} shows a typical example, where the soccer ball is
identified as a frisbee, which is incorrect but still relevant to the ``sport''
theme.
It is hard for the storyline predictor to distinguish these mistaken objects
and appropriate objects, leading to grounding errors.
A better object detector could mitigate this problem; or we can optimize
plotting and generation together, {\em i.e.}, including ``reworking'' in
storyline plotting.


\begin{figure}[htbp]
    \centering
    \includegraphics[width=\linewidth ]{figures/error_analysis.pdf}
    \caption{Grounding error example of {\system}.} 
    \label{fig:error}
\end{figure}

%------------------ dead kitten ----------------

\begin{comment}



We believe error rates can be reduced by improving prediction in the object detection model to predict more appropriate objects.
The other direction is to optimize plotting and generation together



skip these mistaken objects in the Story Graph because, semantically, these objects still fit in the theme.

 the storyline predictor are unable to distinguish ambiguous objects and appropriate objects, leading to grounding errors.



When these ambiguous objects occur in the Story Graph, 




ambiguous objects ({\em e.g.}, \emph{frisbee}, as demonstrated in Figure~\ref{fig:error}). 



the \system and KG-Story's 
The


the least ranked

\system increases the explainability due to multi-stage design, allowing us to examine each stage's limitations.
We calculate the number of six aspects votes for \system and KG-Story's last place stories in qualitative analysis. 
The most-mentioned error, accounting for 24.6\%, is also grounding.

In the story-plotting stage, Faster-RCNN sometimes predicts ambiguous objects ({\em e.g.}, \emph{frisbee}, as demonstrated in Figure~\ref{fig:error}). 
The ambiguous objects are wrongfully detected objects that are semantically related to the overall scenario.
Using objects as input to the storyline predictor and candidate entities, the storyline predictor are unable to distinguish ambiguous objects and appropriate objects, leading to grounding errors.
%Moreover, while story reworking improves overall story quality by
%manipulating the story content, it may ``forget'' to delete story elements
%mispredicted by Faster-RCNN and the storyline predictor; thus the generated stories
%retain ambiguous objects, leading to grounding errors.


% why ploting didn't learn to avoid the error nodes? Because mostly it fits in context and hard to tell it's wrong

\end{comment}


==> origin/ethical-orig.tex <==
\section{Ethical Consideration}
Although our research aims to produce short stories that are vivid, engaging,
and benign, we are aware of the possibilities of utilizing a similar approach
to generate inappropriate text ({\em e.g.}, generating violent, racial, gender
insensitive stories).
The proposed visual storytelling technology enables people to generate stories
rapidly based on photo sequences at scales, which can also be used with
malicious intents, for example, to make up fake stories using real images.
Finally, the proposed methods use external knowledge graphs and, therefore,
could easily inherit the issues, risks, and biases in such information sources.
It will require more research to mitigate these potential risks. 


==> origin/experiment-orig.tex <==

%\ethan{I may delete datasets.}
\subsection{Data Setups}
Four datasets are used in this paper: VIST dataset, Visual Genome, ROCStories,
and AMT Human Ranking.
VIST dataset and Visual Genome are used to construct the knowledge graphs, and 
ROCStories supplies a large quantity of pure textual stories for pre-training
the story generator.
%, and AMT Human Ranking data is used for story evaluator.
VIST dataset is also used in Story-Plotting for training storyline predictor
and in Story-Reworking to fine-tune the story generator.
% \paragraph{VIST}
% We conducted experiments on VIST~\cite{huang2016visual}, which
% includes 10,117 Flicker albums with 210,819 unique images. We followed the
% standard split setting as previous work, with 40,098 samples for training,
% 4,988 for validation, and 5,050 for testing. Each sample contains one story that
% describes five images from a photo stream.
% \paragraph{Visual Genome} Visual Genome~\cite{Krishna_2017} is a
% knowledge-based dataset that connects images concepts to language. It has
% 108,077 images, 3.8 million object instances, and 2.3 million relationships.
% The knowledge graph we utilize covers nouns and relations, categorized
% into semantic frames, provided by the scene graph of Visual Genome.
% % Compared with most image-to-text works that focus on objects nouns and generate static stories, adding logical relation and activities frames makes our stories reasonable and vivid.
% \paragraph{ROC-Stories Corpora} We use the ROC-Stories 
% Corpora~\cite{mostafazadeh2016corpus}, which contains 98,159 pure textual stories, to
% pre-train our story generator.
% As the annotators were asked to write five-sentence stories given a prompt,
% ROC-Stories focuses on specific, everyday topics.
% \paragraph{AMT Human Ranking}
Notably, we also collect MTurk Human Ranking data to train the story evaluator.
We use the ranking results from KG-Story\footnote{Data provided by
authors.}~\cite{hsu2020knowledge}.
This data contains two experiments, each experiments contains 500 distinct
photo sequences. A photo sequence contains a set of machine generated stories
ranked by five MTurk workers. As a result, we collect 5000 data MTurk worker
annotation data. 
Specifically, MTurk workers were asked to rank AREL~\cite{wang2018show},
KG-Story, two KG-Story ablation models, and reference stories, using 3
different settings of their model in each experiment.
We select rank 1 and 5 stories as positive and negative samples. 


\subsection{Baselines}
Several competitive baseline models are chosen. 
\textbf{AREL}~\cite{wang2018show} and \textbf{GLAC}~\cite{kim2018glac} are
end-to-end models with augmentations of reinforcement learning and
global-location attention mechanisms, top rank in VIST
Challenge\footnote{http://visionandlanguage.net/workshop2018/\#challenge}. 
% is an approach based on reinforcement
% learning which learns an implicit reward function with imitation learning for
% story generation.
% 2) \textbf{GLAC}~\cite{kim2018glac} uses Bi-LSTM as encoder and LSTM as
% decoder. It  applies global-local attention and context cascading mechanisms
% that focuse sequentially on the encoder output when generating sentences.
\textbf{KG-Story}~\cite{hsu2020knowledge}, the current state-of-the-art framework, 
utilizes a knowledge graph to 
enrich the story contents
and generates stories using
Transformer.
% \subsubsection{AREL}~\cite{wang2018show} is an approach based on reinforcement
% learning which learns an implicit reward function with imitation learning for
% story generation.

% \subsubsection{GLAC}~\cite{kim2018glac} uses Bi-LSTM as encoder and LSTM as
% decoder. It  applies global-local attention and context cascading mechanisms
% that focuse sequentially on the encoder output when generating sentences.

% \textbf{ReCo-RL} \cite{hu20aaai}: ReCo-RL develops a reinforcement learning policy and learns reward functions designed to increase three criteria: relevance, coherence, and expressiveness, for story generation. \yun{delete if we lose}

% \subsubsection{KG-Story}~\cite{hsu2020knowledge}, a three-stage approach,
% utilizes a knowledge graph to 
% enrich the story contents
% and generates stories using
% Transformer with positional encoding, anaphoric expression generation, and
% repetition penalty.

% \ethan{I think we can replace baselines with AMT data}
% \yun{shrink baseline as one paragraph}

\subsection{Evaluation Methods}

Per literature~\cite{wang2018show}\kenneth{CITE AREL}, human evaluation is the
most reliable manner to evaluate the quality of visual stories, and automatic
metrics often fail to align faithfully to human
judgments~\cite{DBLP:journals/corr/abs-1906-01764}\kenneth{CITE VIST-APE}.
Therefore, in this paper, we prioritize human evaluation over automatic evaluations.

\paragraph{Human Evaluation}
%\ethan{I emphasized on the newly proposed human evaluation result}
A validated VIST autometric is yet to be developed. For evaluation
persuasiveness and authenticity, human evaluation is still preferable. 
%To further evaluate the quality of generated stories, 
We conducted human evaluations through crowd-sourcing Amazon Mechanical Turk
(MTurk) to further evaluate the quality of generated stories. 
%We propose a novel data collection method to obtain more meaningful and resourceful
%and cost-effective 
%human experiment results\yun{can delete, novel questionnaire below}. 
For each experiment, we randomly selected 250 stories, each of which was
evaluated by five different annotators in the US. The experiment includes a
comparison study with three baseline models and three ablation studies, and
each annotator is compensated 0.1 USD for each experiment. 
% \textbf{(1) Quality Ranking:}
The workers were asked to rank the stories (e.g., our story and
baseline/ablation models) based on their overall quality. 
In addition, the user interface also provides a novel questionnaire to collect
in-depth feedbacks from MTurk workers. The questions include ``what do you like
about the best stories'' and ``what do you dislike about the worst stories''
for workers to select aspects that affect the overall story qualities.  
These aspects are provided by \citet{huang2016visual} which includes focus,
coherence, shareability, humanness, grounding, and detail.
% 1) Focus: does the story have a focused topic, 2)
% Coherence: is the story well-structured and grammatically correct,
% 3) Shareability: would the workers like to share the story with their
% friends, 4) Humanness: does the story seem like it was written by a
% human,  5) Grounding:  does the story reflect the entities in the
% images, 6) Detail: does the story contain an appropriate level of
% details. ~\ethan{is this section detailed enough?} \yun{if there's description for each aspect in cited paper, can delete?}
We calculate the average rank and the majority rank among 5 workers for each
story, as well as, each model's total best and worst aspects. 


\paragraph{Non-Classic Automatic Evaluation: BLEURT, voc-d, and MLTD}
%Traditional n-gram-based automatic metrics such as BLEU and METEOR are commonly used in text generation evaluation. 
%However, 
A large set of prior work in VIST have shown that the classic automatic
evaluation scores, , such as BLEU and METEOR, correlate poorly with human
judgments~\cite{hsu2020knowledge, hu2019makes, Wang2020StorytellingFA, Li_2020,
pengchengKnowledge2019, DBLP:journals/corr/abs-1906-01764, wang2018show,
modi-parde-2019-steep}.
%In VIST, 
These n-gram matching metrics fail to account the semantic similarity to the
reference stories and lexical richness in the generated stories. 
%The visual stories are meant to be diverse and detailed, 
%The concerns about reliability of the automatic scores. 
Thus, we adopt BLEURT~\cite{sellam2020bleurt}, a state-of-the-art BERT-based
learned evaluation metric, to further correlate generated stories and reference
stories based on their semantic meaning. Additionally, we also adopt lexical
diversity metrics: voc-d and MLTD~\cite{Lexical} to quantify story lexical
richness. 
% n-gram inter-story repetition rate (\(r_e\)) ~\cite{Lexical} to quantify story lexical richness. 
%The lexical diversity is also important to vivid visual short stories  ~\cite{DBLP:journals/corr/abs-1804-09160},
Several works have shown the lexical diversity are positive correlated to story
quality ~\cite{Liu_2019_ICCV, dai2017towards}. 
%yet negative correlated to n-gram based metrics ~\cite{Liu_2019_ICCV, dai2017towards}. %Several lexical diversity metrics: voc-d, and n-gram inter-story repetition rate \(r_e\), were proposed by
%Most classic n-gram-based metrics analyze the overlap between the
%generated stories and the ground truth, they fail to account for
%meaning-preserving lexical diversity~\cite{DBLP:journals/corr/abs-1804-09160}.
%For example, a thorough story may be given a lower score while a meaningless story
%with only prepositions and pronouns can %be used to 
%get high scores.
%Therefore, we also use other automatic metrics to evaluate stories from
%different aspects.
% However, \citet{DBLP:journals/corr/abs-1804-09160} has pointed out traditional gram-based metrics, which are based on the overlap between the generated stories and the ground truth, fail to account for meaning-preserving lexical diversity.
% Thus relevant story may get a lower score while a meaningless story with only preposition and pronoun has the chance to cheat scores. 
% Therefore, we set up other automatic metrics for evaluate stories in different aspects.
%~\citeauthor{Lexical} and ~\cite{DBLP:journals/corr/abs-1811-05701}. ~\ethan{Yunwei could you provide some more details about MTLD and voc-d?}
%The n-gram inter-story repetition rate \(r_e\) evaluates the diversity of each stories \yun{can site or footnote the paper to save space}.

% The repetition rate \(r_e\) is shown in Equation ~\ref{repetition}, 
% \begin{equation} 
%     r_e = 1 - \frac {|\sum_{i=1}^{N} \sum_{j=1}^{m} f_{n}^{*}(y_{i,j})|}{\sum_{i=1}^{N} \sum_{j=1}^{m}|f_{n}(y_{i,j})|},
% \label{repetition}
% \end{equation}

% where \(y_{i,j}\) represents the $j$-th sentence of the $i$-th story,
% \(f_{n}(\cdot)\) returns the set of n-grams of the sentence,
% \(f_{n}^{*}(\cdot)\) returns the distinct set of n-grams, and \(|\cdot|\) is
% the number of elements in a set. 
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth ]{figures/big_figure1.pdf}
	 \caption{Generated stories for \system and baseline models. MTurk workers
	 were asked to rank the stories. 
	 %with a {\system} storyline
	 %displaying the ingredients of generated story. For {\system}, words in blue
	 %indicate story elements and words in red are semantic frames predicted
	 %after storyline prediction.
	 }     
    \label{fig:baseline_comparison}
\end{figure}




% \textbf{(2) Aspects Rating:} Given a sequence of images and its corresponding story, workers are asked to choose the degree of agreement from 1 to 5 for 7 different aspects provided by VIST.
% These aspects include: \textcircled{1} Focused: If the story has a focused topic, \textcircled{2} Coherent: If the story is well-structured and grammatically correct, \textcircled{3} Share: If the workers would like to share the story with their friends, \textcircled{4} Human: If the story seems like it was written by human,  \textcircled{5} Grounded:  If the story reflects entities in the images, \textcircled{6} Detailed: If the story contains appropriate level of details, \textcircled{7} Entertaining: If the story is interesting or entertaining.
% \yun{change if we do not put 7aspect, bottoms for 7 aspect}




==> origin/human-eval-result-orig.tex <==


%\subsection{Qualitative Analysis} 
%For the qualitative analysis, 
%In this work, 
We ask MTurk\kenneth{let's use MTurk instead of AMT}\yun{solved} workers to
rank four stories, {\em i.e.}, the \system's and three baseline models',
including that of the state-of-the-art KG-story. 
Table~\ref{tb:human_ranking} shows the results.
\system outperforms other models in average ranking: it outranks AREL by 0.24
and KG-Story by 0.16. 
As for the percentage of 1st-rank stories, \system produces 12.0\% more than
AREL and 7.5\% more than KG-Story.
%, having 12.0\% more ranked 1st stories than AREL; ranks better by 0.16, having 7.5\% more ranked 1st stories than KG-Story. 
Figure~\ref{fig:baseline_comparison} shows an representative example.
Compared with end-to-end models ({\em i.e.}, AREL and GLAC), graph-based
methods ({\em i.e.}, KG-Story and \system) generate more diverse stories.
%, whereas AREL and GLAC generate repetitive, general sentences ({\em e.g.}, ``there were a lot of/many people there''). 
Compared with KG-Story, whose sentences are relatively simple and plain, such
as ``many people showed up'', our model reuses entities such as \emph{parade}
in the first sentence and associates relations with other entities, {\em e.g.},
\emph{people} and \emph{runners}, to compose ``many people showed up to watch
the parade runners''. 
Thus, \system yields better story quality in terms of coherence and detail. 
%They questionnaire also allows us to conduct more in-depth analysis on our proposed model's strength and weakness by reviewing feedbacks for highest ranked stories and lowest ranked stories. 
Moreover, Figure~\ref{fig:ours_kgstory_bar2} shows the questionnaire result for
the best-ranked stories.
For {\system} and KG-Story's best-ranked stories, the {\system} story count is
significantly higher in all aspects; specifically, coherence, shareability, and
humanness are higher than other categories.

%Since KG-Story only uses additional 1 relation among 5 images, it probably will generate caption-like sentence (e.q., it was a nice car.) for the image without any relation linked.
%\yun{with the help of storyline....sale organize and coherence(runners)}
\input{tables/baseline_rank}
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth ]{figures/histogram.pdf}
	 \caption{Number of six aspects votes for {\system} and KG-Story's first
	 place stories. \system significantly outperforms in coherence, humanness,
	 and grounding.
} 
\label{fig:ours_kgstory_bar2}
\end{figure}


%This shows the advantage of story plotting, and story reworking for visual storytelling. 
%\ethan{FIGURE}


%In Table ~\ref{tb:human_ranking}, it displays the ranking distribution of \system with three baseline models (AREL, GLAC and KG-Story). ~\ethan{KG-Story or KG-Story...consistence.} 



%\yun{win A model, win B model...7-asepct, diversity, repetition, across images, length}
%\ethan{aspect, amount of good stories, figure to explain, without...ablation study}




%\yun{of course the difference between PRE-VIST & w/oRE is big cause RE is designed by human-judgement, the function of RE is to refine the story and check the grammar (like a teacher), but it did not control the writing ingredient, but we dig deep into the the data in w/oPE, P control the writing ingredient, (1) manage nouns for generator (2) make sentence vivid(use figure)}




==> origin/introduction-orig.tex <==
\section{Introduction}

\begin{figure*}[t]
    \centering
    %\includegraphics[width=\linewidth]{figures/flowchart_cam2.pdf}
    %\includegraphics[width=\linewidth]{figures/new_flowchart.pdf}
    \includegraphics[width=\linewidth]{figures/overview.png}
    %\vspace{-1.5pc}
	\caption{Overview of {\system}. \textbf{Preparation}: %The nouns and verb frames of the stories in VIST-dataset are transformed in to VIST-Graph.  
	Extracting $objects$ and $terms$ from the images as entities, verb frames
	from VIST and VG-Graph as edges, we create a story graph for the images.
	\textbf{Story-Plotting}: Finding a path from
	\texttt{$<$s{\scriptsize{i}}$>$} to \texttt{$<$s{\scriptsize{i+1}}$>$} as an
	event, the predictor collects a sequence of  events to develop a storyline.
	\textbf{Story-Reworking}: A story generator generates the story according to
	the storyline. 
	}
	\label{fig:flowchart}
    %\vspace{-1pc}
\end{figure*}


Writing a story is a complicated task.
Human writers use their knowledge to tie all the disjointed elements, such as
people, items, actions, or locations, together to form a coherent storyline.
Writers also re-evaluate their work constantly when they are writing, and
sometimes even alter their writing goals in the middle the draft.
\citet{flower1981cognitive} characterized a solo writer's cognitive process as
a series of components, in which the writer's own knowledge is described as the
``Long-Term Memory'';
and the planning, translating, and reviewing steps can occur in an
``recursive'' and ``interconnected'' manner in the Writing Processes.
These creative steps are essential to human's writing.
On the other hand, however, automated visual storytelling (VIST) models that
compose stories given five images~\cite{huang2016visual}, 
do not make extensive use of human knowledge to tie all the elements,
nor use human insights to evaluate the outputs and guide the generation process.

%rework the generated text to iteratively improve the story.
As for linking elements, most prior works generated visual stories in an
end-to-end fashion~\cite{huang2016visual,kim2018glac}, treating this task as a
straightforward extension of image captioning.
Several recent work started using relations between entities to improve visual
storytelling, but often narrowed in on a particular subset of relations, such
as 
relations between elements within the same image\kenneth{TODO: ADD REFERENCE},
relations between two adjacent images~\cite{hsu2020knowledge}, or 
relations between scenes~\cite{Wang2020StorytellingFA}.
The full potential of rich real-world knowledge and complex intra-image
relations have not been fully utilized.
As for re-evaluating, some recent work used reward
systems~\cite{DBLP:journals/corr/abs-1804-09160,hu2019makes} or estimated topic
coherence~\cite{wang2019consistent} to asses the output story and guide the
generation process.
However, these approaches often optimized towards a predefined aspect, such as
image relevancy or topic coherence, which do not necessarily result in a
high-quality or engaging story from human's perspectives.
The writer's judgements are critical in the cognitive process of human writing,
and visual storytelling models might benefit from considering human ratings.



This paper introduces \textit{\textbf{\system}}, a novel visual storytelling
framework that first constructs a graph the captures the relations between all
the elements in the input image sequence,
finds the optimal path in the graph that forms the best storyline,
and uses the found path to generate the story.
Figure~\ref{fig:flowchart} overviews \system.

\begin{itemize}
	 \item \textbf{Stage 1 (Story Plotting):} \system first constructs a ``Story
	 Graph'' for the image sequence by extracting various elements ({\em i.e.,}
	 term nodes, object nodes) from all the images and linking these elements by
	 using external knowledge ({\em i.e.,} VIST graph, VG Graph). \system then
	 finds the ``best path'' in the Story Graph as the ``storyline'' and feed it
	 to Stage 2.

\item \textbf{Stage 2 (Story Reworking):} \system uses a story generator and a
story evaluator to realize the ``rework'' process: the generator takes the
storyline produced in Stage 1 as the input to generate the story and
back-propagates with evaluator-augmented loss function. 
The evaluator, a discriminator model trained on human rating score data to
classify good and bad stories, outputs a story quality score and modifies the
loss. 
After a few optimization epochs, the generator eventually learns to generate
stories that 
%, in which the writing style 
%finally %eventually 
reflects human preferences.%\kenneth{So the iterative process will not occur in testing time? This part needs to be more clear.}
%The process of back-propagation is an analogy 

%In this paper, a storyline is a sequence of nouns and verb frames.
\end{itemize}


In \textbf{Stage 0 (Preparation)}, a set of knowledge graphs that encode
relations between elements should be prepared for the uses in Stage 1 and
training.
In this work, we prepare two knowledge graphs: the VIST Graph and the Visual
Genome (VG) Graph. 
We construct the VIST Graph based on the VIST dataset, representing the
in-domain knowledge; and VG Graph is an existing resource~\cite{Krishna_2017},
representing generic knowledge.
Note that the \system framework is generic so it can use any knowledge graphs as needed.
%Both graphs contain comprehensive visual and story relations, namely, noun-verb-noun (NVN) interactions. 
%Then, the detection models extract the story elements: objects and terms from each images. %, describing complex story elements interactions of five images.

The automatic and human evaluations show that \system produces visual stories
that are more diverse, coherent, and human-like.
We also conduct an ablation study to show that both story plotting (Stage 1)
and reworking (Stage 2) contribute positively to the model's superiority.
%advance in diversity, coherence, and humanness, per both automatic and human evaluations.
%The ablation study shows that both plotting and reworking contribute to the model's superiority.
We believe this work also shows the potential of drawing inspirations from
humans' cognitive processes or behaviors to improve text generation
technologies.






%------------------------- dead kitten ----------------------------------------

\begin{comment}

The contribution of this paper are 4-fold.
First, we propose \system, a novel framework that organizes story elements, models storylines, and reworks the story to perfect the story. 
Second, we propose novel knowledge graphs to associate story elements and increase
coherence between images with visual and story intuition.
Third, we propose modeling storylines by organizing story elements via relation
extraction over the knowledge graph. 
%The plotted storyline outlines a reasonable story flow for image stream. ~\ethan{outline or sketch?}
Fourth, we enable the usage of various human story evaluation results 
%for different models %
%under different settings 
in the reworking phase to refine our stories.
%with human judgement, thus, the generates stories are aligned to human preference. 
%~\ethan{pls refer to Question 3, Question 6}


%\ethan{
%Questions:

%1. just a draft, need to be fixed.
%LWKU: please fixed it now.

%2. Should we mention our recurrent structure and hierarchical loss in the introduction
%LWKU: if you can link them well to the two major points.

%3. The contribution sounds a bit weak, should we be more descriptive? e.g. state the advantage of multi-aspect graph. 
%LWKU: Let me do this.

%4. A relation extractor pops out of nowhere, it's a bit unexpected, should I mention relation extractor in that sentence? 
%LWKU: use another term to abstractively describe it.

%5. We've decided to name two types of visual elements (visual and story intuition) as implicit and explicit visual elements, however, please feel free to propose and edit the name. 
%LWKU why not just use visual and story? More straightforward.
%6. We also have a few other additional advantages: diversity, framework output transparency (we know exactly what we're inputting to the story generator), diverse length (recurrent transformer). We may add those advantages in the later edition, if and only if it does not diverge the focus. Any suggestions as to where to add them? Intro, Evaluation, Mythology? Or don't add them at all? 
%LWKU: discussions together with the evidence which supports them?

%7. We've decided to name the subgraph as relation graph instead of image graph or story graph. Feel free to propose and edit the name. 
%LWKU: sounds good. If relation does not to be emphasized, maybe plot graph?
%}
% \ethan{Note: I used a lot of image Stream, make sure to make connection between image sequences and image stream LWKU: what is an image stream? represent 5 images}



%\ethan{
%1. multi aspect knowledge graph 

%a. Diversity 

%b. visual and story (implicit and explicit visual elements) nouns: VIST-Graph, story noun prediction, visual and story relations

%2. Plotting: novelty, none of the work use path searching, within-across image relation, comprehensive view. arrange a story flow by learning ground-truth stories, coherent. 

%3. Generation:

%a. Diverse input, Hierarchical

%c. Utilize AMT data.  Reward Function

%}
%The story editing stage consisits a story generator and a rating system to generat a story and update the generated story according iteratively. 





% \begin{figure*}[t]
%     \centering
%     \includegraphics[width=\linewidth]{figures/fig1.pdf}
%     \caption{(a) ...need adjust...red nodes are $N_{story}$ from story-noun extractor (b)From the human-written stories of VIST training data, we build a VIST-Graph with reading direction.}   
%     \label{fig:flowchart}
% \end{figure*}


The objective of visual storytelling (VIST) is to automatically compose a story given five images~\cite{huang2016visual}.
Similar to image captioning~\cite{Fang_2015}, a visual story must be descriptive and relevant to the images. 
VIST, however, further demands the visual stories be well-composed into cohesive and appealing sentences. 
%Inspiring from human story writers, we structure storytelling into plotting, and re-editing. 
%To attain human-level visual story writing, %this paper adopts 
For human writers, two writing skills are applied to improve story writing:
\textit{story-plotting} and \textit{story-reworking}~\cite{stephenking_edit,
 jamesscottbell_plot}, which reworking is inclusive of writing and editing. 
%Plotting and re-editing are arguably the most important components . 
%Intuitively, plotting a storyline helps because it allows us to step back and get a broader view of the narrative. Reworking also helps because it gradually improves the story quality by revising and refining repeatedly. 

 %. The subjective assumptions of a ``good story'' can diverge from human judgement. 
%While good story, they alter the story style \ethan{?} depending on their pre-defined autometrics.
%\lwku{what do you mean by subjective definition?}
%However, most knowledge graph based studies only considered uni-directional relation, and very little works researched in plotting a complete storyline from the visual elements.
%However, most knowledge graph based considered 
%While all of the studies showed their experiment result by conducting human evaluation on AMT (Amazon Mechanical Turks), none of the studies reuses the human evaluation results .
%\lwku{this is awkward here} \ethan{saw your edit, is this still awkward?} Although prior story editing studies demonstrate various approaches for VIST, 
%While all visual storytelling researches conducted human evaluations on AMT (Amazon Mechanical Turks) and received valuable human annotation data, 
%most visual storytelling researches conducted story ranking evaluations on Amazon Mechanical Turks (AMT) to examine the proposed methods, and received valuable human annotated results. 
%This paper, on the other hand, proposes an innovative approach to reuse the story ranking evaluation result, achieving an objective story writing refinement. %~\ethan{, aligning to human preference.}
%valuable Amazon Mechanical Turks (AMT) human evaluation annotations. 
%However, very little works have researched in plotting a complete storyline from the visual elements, nor utilizing prior studies' human evaluation data in reward system.

%Inspired by prior studies ~\cite{hsu2020knowledge, Wang2020StorytellingFA}, we converted the visual elements to 

%We analogy the path searching task in knowledge graph as story plotting stage; a reward score embedded story generator as story editing stage. ~\ethan{need to rephrase}


%Visual storytelling ~\cite{huang2016visual} is characterized as a vision-to-language task. %, which the goal is to write a story from a sequence of images. 
%Similar to image captioning ~\cite{Fang_2015}, it requires an automation method to compose a textual description from images. While most image captioning studies focus on image and caption's relevence \ethan{citation}, VIST distinguish itself by including story coherence, 



%achieving an objective story writing refinement.
% after the editing cycle.
%~\ethan{please refer to Question 2. }

%did not receive human insight for guidance 
%they may unalign to human judgement.
%This paper on a storytelling dataset, VIST,  ~\cite{huang2016visual}, which the goal was to compose a story given five images. 
%Recent VIST studies reveal two obstacles in attaining human-level writing.
%Recent VIST studies attempt different approaches to attain human-level writing. 
% by improving the image relevancy and story coherence. 
%To improve image relevancy, current works modified RNN to learn image features ~\cite{kim2018glac}. Other works
While most studies improve image and story coherence by associating cross-image
entities, previous graph-based approaches
%Some approaches increased story and image coherence by associating cross-image entities among five images. Graphical neural networks perform cross-image object associations before story generation \cite{Wang2020StorytellingFA}. 
%Knowledge graphs are also utilized to find a single cross-image relation between two adjacent images~\cite{hsu2020knowledge} to enrich story content. 
%, thus, it provides a connection sentence to cohere the story. 
%On the other hand, 
 %Thus, %it maintains subject consistency throughout the story. 
%However, %the current end-to-end model still produce monotonous stories with low lexical diversity\lwku{awkward sentence}. The 
%previous graph-based approaches %barely plot a complete storyline, as they
% only consider partial cross-image associations. They
do not fully utilize real-world knowledge or intra-image relations ~\cite{Wang2020StorytellingFA,
hsu2020knowledge}, 
%nor do they comprehensively associate and organize every image entities,  
%thus, they are unable to fully utilize the knowledge\lwku{why?}, 
limiting the potential to exploit the knowledge. % to compose coherent stories.
%\ethan{fixed}
%generated are still fall far behind human written stories. Thus, %none of the graphical studies constructed an well-defined relation graph that conveys complex inner-intra entities relations throughout the entire image stream. \ethan{pls refer to Question 1} %have designed a cross-image graph to connect the image steam
%Nor searching and utilizing intra-inner image relations, which we define the searching process as story plotting. \yun{path searching} %The model effectively reuses objects across images to improve story coherence. 
%\ethan{relation graph???image graph???} %across images. %~\ethan{?? and what is missing in the current study...rephrase, reuse and connect, and arange}
Implementing topic-coherence ~\cite{wang2019consistent} or
reward systems~\cite{DBLP:journals/corr/abs-1804-09160, hu2019makes} are helpful in their target criteria. However, these approaches
only %modify the story generation process based on pre-defined aspects. That is,
%optimizing 
optimize the generation model towards specific aspects, such as image relevancy or topic coherence, and they may unalign to human judgement.






%increase the language-vision coherence by associating cross-image entities among all images~\cite{Wang2020StorytellingFA,hsu2020knowledge}
%Implementing topic-coherence~\cite{wang2019consistent} or reward systems~\cite{DBLP:journals/corr/abs-1804-09160, hu2019makes} are helpful in their target criteria.

%As human visual story writers, we observe the images, organize the visual elements, and write a story. For some dedicated writers, they even seek for a third party opinion to edit and refine their writing style. ~\ethan{need to rephrase}
%the written story.
%Our proposed framework, \system, is motivated by such systematic story writing process. 
%Inspired by prior studies ~\ethan{be specific}, 
To this end, we introduce {\system}, a novel visual storytelling framework that
plots a storyline outlining five images and writes a story accompanying with a reworking process. %through an iterative reworking process. 
% utilize the knowledge graph \yun{to ...} and relation extraction model for storyline plotting, as well as, \yun{another sent}reusing prior research's AMT human evaluation data to rate and refine the writing style. 
This framework consists of preparation stage and two story-writing stages: story-plotting and story-reworking, as
demonstrated in Figure~\ref{fig:flowchart}.
In the preparation stage, we prepare two knowledge graphs: VIST Graph and Visual Genome (VG) Graph, containing comprehensive visual and story relations, namely, noun-verb-noun (NVN) interactions. Then, the detection models extract the story elements: objects and terms from each images. %, describing complex story elements interactions of five images.
In the story plotting stage, the images in a story is transformed into a graph, named story graph. All extracted story elements in five images are linked altogether by using verbs in the knowledge graphs. The storyline predictor pathfinds a storyline in the story graph, that is, the story predictor selects multiple relations that are appropriate for storytelling. The output storyline is a sequence of nouns and verb frames.
%\lwku{check verbs}. %For each image, the system extracts two sets of elements: image and story oriented visual elements. 
%The image oriented visual elements are image objects and story oriented visual elements are inferred information such as events.~\ethan{fixed}
%The explicit visual elements represent visual intuition. %, which contains obvious objects that can be easily detected by object detection models. The implicit visual elements represent the story intuition that can be inferred from the image, such as events, dates, or locations. \ethan{pls refer to Question 5.}
%Pairing two story-nouns, we u
%To obtain the relations between story-noun , we utilize a visual and a story common-sense knowledge graph to extract the relations between story-nouns.
%depicting object interactions in images and stories, are used to link the extracted story-nouns. 
%to another in the visual element graph, until the storyline reaches an appropriate length. 
%~\ethan{pls refer to Question 4} %Unlike ~\cite{Wang2020StorytellingFA}
%The relation extraction model is used to distills and arrange the story-nouns, as well as, narrates and outlines the story flow of the given images. 
%the system observes and extracts the visual elements from the images. Using object detection 
%\ethan{is reworking actually appropriate, it is essentially back-propagation}
The story reworking stage consists of a story generation model and a story evaluator. The generation model uses the storyline as the input to generate the story and back-propagates with evaluator-augmented loss function. 
%The generation model takes storyline as the input to generate stories. 
The evaluator, a
discriminator model trained on human annotation data to classify good and bad stories, outputs a score and modify the loss. %The reward score is augmented with Maximumlikelihood estimation (MLE), so that the model can be optimized to a more human-like model
%\yun{too detail}.
%That is, the reward score is used to modify the MLE value.
%The story generator then edits the story according to the reward and returns the
%revised story to the reward system. 
After a few optimization epochs, the model can generates an optimal refined story, in which the writing style eventually
reflects human preferences. %The process of back-propagation is an analogy of iterative reworking process.
%Although prior story editing studies demonstrate various approaches for VIST, 


The story reworking stage consists of a story generation model and a story evaluator. 


The generation model uses the storyline as the input to generate the story and back-propagates with evaluator-augmented loss function. 
%The generation model takes storyline as the input to generate stories. 
The evaluator, a
discriminator model trained on human annotation data to classify good and bad stories, outputs a score and modify the loss. %The reward score is augmented with Maximumlikelihood estimation (MLE), so that the model can be optimized to a more human-like model
%\yun{too detail}.
%That is, the reward score is used to modify the MLE value.
%The story generator then edits the story according to the reward and returns the
%revised story to the reward system. 
After a few optimization epochs, the model can generates an optimal refined story, in which the writing style eventually
reflects human preferences. %The process of back-propagation is an analogy of iterative reworking process.
%Although prior story editing studies demonstrate various approaches for VIST, 



In the story plotting stage, the images in a story is transformed into a graph, named story graph.
All extracted story elements in five images are linked altogether by using verbs in the knowledge graphs.
The storyline predictor pathfinds a storyline in the story graph, that is, the story predictor selects multiple relations that are appropriate for storytelling. The output storyline is a sequence of nouns and verb frames.





At the testing time, 

This framework consists of preparation stage and two story-writing stages: story-plotting and story-reworking, as
demonstrated in 




plots a storyline outlining five images and writes a story accompanying with a reworking process. %through an iterative reworking process. 
% utilize the knowledge graph \yun{to ...} and relation extraction model for storyline plotting, as well as, \yun{another sent}reusing prior research's AMT human evaluation data to rate and refine the writing style. 

In the preparation stage, we prepare two knowledge graphs: VIST Graph and Visual Genome (VG) Graph, containing comprehensive visual and story relations, namely, noun-verb-noun (NVN) interactions. Then, the detection models extract the story elements: objects and terms from each images. %, describing complex story elements interactions of five images.
In the story plotting stage, the images in a story is transformed into a graph, named story graph. All extracted story elements in five images are linked altogether by using verbs in the knowledge graphs. The storyline predictor pathfinds a storyline in the story graph, that is, the story predictor selects multiple relations that are appropriate for storytelling. The output storyline is a sequence of nouns and verb frames.
%\lwku{check verbs}. %For each image, the system extracts two sets of elements: image and story oriented visual elements. 
%The image oriented visual elements are image objects and story oriented visual elements are inferred information such as events.~\ethan{fixed}
%The explicit visual elements represent visual intuition. %, which contains obvious objects that can be easily detected by object detection models. The implicit visual elements represent the story intuition that can be inferred from the image, such as events, dates, or locations. \ethan{pls refer to Question 5.}
%Pairing two story-nouns, we u
%To obtain the relations between story-noun , we utilize a visual and a story common-sense knowledge graph to extract the relations between story-nouns.
%depicting object interactions in images and stories, are used to link the extracted story-nouns. 
%to another in the visual element graph, until the storyline reaches an appropriate length. 
%~\ethan{pls refer to Question 4} %Unlike ~\cite{Wang2020StorytellingFA}
%The relation extraction model is used to distills and arrange the story-nouns, as well as, narrates and outlines the story flow of the given images. 
%the system observes and extracts the visual elements from the images. Using object detection 
%\ethan{is reworking actually appropriate, it is essentially back-propagation}
The story reworking stage consists of a story generation model and a story evaluator. The generation model uses the storyline as the input to generate the story and back-propagates with evaluator-augmented loss function. 
%The generation model takes storyline as the input to generate stories. 
The evaluator, a
discriminator model trained on human annotation data to classify good and bad stories, outputs a score and modify the loss. %The reward score is augmented with Maximumlikelihood estimation (MLE), so that the model can be optimized to a more human-like model
%\yun{too detail}.
%That is, the reward score is used to modify the MLE value.
%The story generator then edits the story according to the reward and returns the
%revised story to the reward system. 
After a few optimization epochs, the model can generates an optimal refined story, in which the writing style eventually
reflects human preferences. %The process of back-propagation is an analogy of iterative reworking process.
%Although prior story editing studies demonstrate various approaches for VIST, 

an NLP task that aims to compose a short story given five images~\cite{huang2016visual}, however, 
do not model 


fully use external knowledge 

nor the iterative editing process.

%\ethan{

%VIST introduction
%What is VIST? Why is VIST important? 

%Unlike image caption, how? 
%Image captioning focuses on generating a descriptive text to describe object relation in an image. VIST: 
%not only it has to describe the relationship between objects, it also make connection between the explicit object and the implicit information, such as festivals, events, or locations. 
%Also, the stories are to describe a consecutive set of events, thus, the stories make connections across images. 

%Use a series of image stream, VIST wanted to generate

%VIST-KG introduction

%kg-story --only inserts a relation

%scene-graph-- unable to walk back

%VIST-RL introduction
%--yunwei

%our works motivation

%first stage -
%graph construction,
%sub-graph construction

%second stage -
%story generation, story editing


%}
% \begin{figure}[t]
%     \centering
%     \includegraphics[width=\linewidth ]{acl-ijcnlp2021-templates/figures/flowchart_cam.pdf}
% 	 \caption{overview of {\system}. \textbf{Stage 1: Story Plotting}: 
% 	 Two types of visual elements are extracted from images and then associated 
% 	 to form a relation graph. A storyline predictor then plots a sequence of
% 	 events into a storyline.
% 	 \textbf{Stage 2: Story Reworking}: By inputting a storyline, a story
% 	 generator accompanied with a story evaluator constantly generates and
% 	 evaluates the story. 
% 	 \yun{pre-writing, stage1, stage2; think upper left; story loss/modified loss; or higher-level concept(more details and a 2 column figure)}
%     %After epochs of editing, the refined story is generated. 
%     %\ethan{I don't think we need Vi and Vs, and Multi-Aspects Knowledge Graph should be capitalized, and I think we could use real example for storyline.}
%   }
%     \label{fig:flowchart}
% \end{figure}

%In recent vision-to-language tasks, there has been an interest in studying image understanding and textual generation.
%Composing a descriptive text from an image or a sequence of images 

%Visual storytelling ~\cite{huang2016visual} is characterized as a vision-to-language task, which the goal is to write a story from a sequence of images. Early studies mainly focus relevancy and descriptiveness ~\cite{kim2018glac}, recent studies have tackled several additional criteria in visual and textual aspects. To cohere the visual elements, several works has consider intra-image relation ~\cite{Wang2020StorytellingFA, }%In visual aspect, it requires intra-image connections, and implicit objects understanding. In textual aspect, the sentences have to be diverse, coherence, detailed and grammatically correctly.
 %For the reason above, we argue story plotting and story editing can improve the story quality ~\ethan{adj, rephrase needed}. %beneficial to structuring visual storytelling. Thus, they improve story quality. %The structured design increases the explainability due to its trans they improve story quality.
% \ethan{keep verb and adjective consistence, extracts, associates, organizes. }

\end{comment}



==> origin/methods-orig.tex <==
%\section{Methodology}

%In the data pre-processing step, in each stories, five images are transformed into a story graph. 
%In the story plotting stage, the framework searches for a path, or plots a
%storyline, to select and arrange the story elements, providing an outline
%for story generation. 
%In the story reworking stage, the story generation model generates a story from a storyline, trained with a discriminator augmented loss function. 

%writes a preliminary story
%from a storyline. This is followed by a story evaluator to  
%an discriminator to 
%rate the generated story, given which the story generator refines the generated stories
%repeatedly. 
%\yun{METHOD: (1) Pre-processing section: a. multi-aspect graph construction, b. story elements extraction, c. "story graph" linking; (2)PR-VIST: story plotting; (3)PR-VIST: story reworking}
%~\ethan{need to be clear...er?} 
%Preparatory to our two-stage framework, w
%For preparation, the framework constructs a multi-aspect knowledge graph conveys visual and story intuition. 
%In the first stage, story plotting, we distil a relation-graph based on constructed multi-aspect knowledge graph that connects five images. 
%We then introduce relation extraction method and plot a storyline on the story-graph.
%The second stage, story editing, introduces generating stories from storylines by story generator and editing stories based on a human-judgment reward function. \yun{need to be edited}
\section{Stage 0: Preparation} 
%In VIST-data, a story is accompanied with five images. 

The preparations for story-plotting is to collect information from the images
and knowledge from the knowledge graphs. 
%: story elements extraction and knowledge graphs construction. 

%design a three-steps procedure for images-to-graph transformation, in which, each set of images is transformed into a story graph: a graph densely displays NVN interactions in within and across the images. 
%using story elements and knowledge graphs. 
\subsection {Story Elements Extraction} 
%Open-SESAME to obtain subject-frame-object tuples. 
%The first step to visual story plotting is gathering all possible information
%from the given five images. That is, we use prediction models to collect visual
%elements and construct a densely connect relation graph to describe complicated
%relations among the five images. 
%among story elements. 
%In an image steam, 
%Each image has a set of story elements extracted by models. 
%In VIST-data, a story is accompanied with five images. 
To extract information from the images, two extraction methods were used to
extract image-oriented and story-oriented story elements: $objects$ and
$terms$, representing image and story intuition.
%\begin{description}
%\item[$\bullet$ Image-oriented story elements ($object$) ] 

\paragraph{Objects} \(objects\) can be detected by current object detection
models, for which we use a pre-trained object detection
model---Faster-RCNN~\cite{ren2015faster}. To ensure detected objects'
reliability, only those objects with the top five of confidence scores are used
in each image.
%\item[$\bullet$ Story-oriented story elements ($terms$)] 
\paragraph{Terms} \(terms\) are story-like noun such as events, time, and
location, which current object detection models are unable to extract.
Therefore, we further use a Transformer-GRU \cite{hsu2020knowledge} to predict
story-like terms. For each images and story pair, we use image objects as the
input and the nouns in the corresponding human-written story as the
ground-truth. The Transformer-GRU learns to convert image features to nouns
that are commonly used in the story.
%\end{description}

%We use the story elements in the image sequence to extract a story graph \(\mathcal{G}_{story}\) from the multi-aspects knowledge graph \(\mathcal{G}_{multi}\) to represent these 5 images. 
%Specifically, the story graph is a sub-graph of the multi-aspects knowledge graph, namely \(\mathcal{G}_{story} \subseteq \mathcal{G}_{multi}\). 


%To train the story-noun predictor, we extract nouns from human written stories also by using spacy.
%The image representation of \(N_{object}\) is fed into a Transformer encoder \cite{vaswani2017attention} and a GRU \cite{chung2014empirical} decoder with attention mechanism \cite{bahdanau2014neural} to generate story-noun \(N_{story}\).
%Additionally, given the VIST dataset has only five images for each story, an image
%position $p \in \{1, ..., 5\}$ is recorded for each $object$ and $terms$ to
%denote their structural relation.
%to denote which image this noun comes from. 
%was dataset that includes desnse interactions and relationships between objects in an image. 
%After extracting \(V_{explicit}\) and \(V_{implicit}\), a
\subsection{Knowledge Graphs Preparation}
To collect interactive relations between nouns,  %$object$ and $terms$, 
we propose Visual Genome Graph  (\(\mathcal{G}_{\mathit{vg}}\)) and VIST-Graph
(\(\mathcal{G}_{\mathit{vist}}\)). 
%multi-aspect knowledge graph \(\mathcal{G}_{\mathit{multi}}\), a large scale graph contains interlinked
%real-world objects and events, displaying SVO interaction
%structures.
These graphs contain interlinked real-world objects and terms, displaying
visual and storytelling interaction.
%structures.
%implicit and explicit knowledge from an image.  Explicit story elements are the objects that can be detected by current object detection model, such as, we implemented Faster-RCNN ~\cite{ren2015faster} to capture the obvious objects. Implicit story elements are the inferred information in an image
%\(\mathcal{G}_{\mathit{multi}}\) is assembled by two proposed graphs: Visual Genome Graph (\(\mathcal{G}_{\mathit{vg}}\)) and VIST-Graph (\(\mathcal{G}_{\mathit{vist}}\)), 
%to obtain visual and storytelling interactions. %\(\mathcal{G}_{\mathit{multi}} =
%\mathcal{G}_{\mathit{vg}} \cup \mathcal{G}_{\mathit{vist}} \)

%\begin{description}
%\item[$\bullet$ Visual Genome Graph (\(\mathcal{G}_{\mathit{vg}}\)) ]
\paragraph{Visual Genome Graph}
{\(\mathcal{G}_{\mathit{vg}}\)} describes pairwise relationships between
objects in an image, describing visual interactions. 
%Excluded the prepositional relations in the original Visual Genome dataset ~\cite{Krishna_2017},
%{\(\mathcal{G}_{\mathit{vg}}\)} provides highly diverse verbal interactions\yun{can delete}.
No prepositional relations are included; only the verbs relations are
preserved. All relations are converted into semantic verb frames by
Open-SESAME~\cite{swayamdipta17open}, in which the semantic frames were
pre-defined in FrameNet~\cite{baker1998berkeley}.   
%Meanwhile, all the preposition relations of VG %\(\mathcal{G}_{vg}\).
%\item[$\bullet$ VIST Graph (\(\mathcal{G}_{\mathit{vist}}\)) ]
\paragraph{VIST Graph}
\(\mathcal{G}_{\mathit{vist}}\) is proposed to collect the storytelling
interactions. We develop this novel story knowledge graph
%depicting entities interaction in VIST \cite{huang2016visual} dataset. 
by converting references in VIST training and validation
dataset~\cite{huang2016visual} to
graphical data. 
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth ]{figures/vist-graph.pdf}
	 \caption{From the stories in VIST training data, a story is transformed a
	 golden storyline following human reading direction, as part of the
	 VIST-Graph.}
% 	 \vspace{-15pt}
    \label{fig:vist-graph}
\end{figure}
%In addition to Visual Genome, we also included storytelling noun interaction to complement visual object interactions. 
%VIST-Graph \(\mathcal{G}_{vist}\) by converting the human-written stories of VIST dataset ~\cite{huang2016visual} to a graphical data. 
Following the reading direction, in each reference, we extract nouns and
semantic verb frames using SpaCy\footnote{SpaCy: https://spacy.io/} and
Open-SESAME to obtain NFN tuples. 
Using nouns and semantic verb frames as nodes and edges, these are collectively
assembled into a golden storyline. 
% ~\ethan{I think \(\mathcal{G}_{xxx}\) is uncomfortable to read.}
%The \((h, r, t)\) is denoted as the head entity, relation, and tail entity respectively.
For example, for ``first pitcher thrown for the game'' in   % AMH: edit Fig.2: pitcher --> pitch %ethan should be pitcher
Figure~\ref{fig:vist-graph}, we extract \emph{pitcher}, \emph{game}, and
\emph{Cause\_motion}, which is a semantic verb frame for \emph{thrown}, as a
NFN tuple.
Additionally, we include a noun token \texttt{$<$s{\scriptsize{i}}$>$} as the
transition point to the next sentence or termination point of a story, and a
verb frame token \texttt{empty\_frame} to interlink two nouns when a semantic
frame is absent. As last, all of the golden storylines are assembled into
\(\mathcal{G}_{\mathit{vist}}\).



\section{Stage 1: Story-Plotting}
\subsection{Storyline Predictor}

In Stage 1, \system uses a storyline predictor to find the ``best path'' in the
Story Graph as the ``storyline'' and feed it to Stage 2.
%The storyline predictor storytells a storyline. 
For the storyline predictor, we select a non-exhaustive relation extraction
framework, UHop~\cite{chen2019uhop}.
%, due to its low computation mechanism in pathfinding.
As a single hop is defined as searching from one entity to another entity by a
single relation.
UHop performs multiple single-hop classifications consecutively in the graph to
pathfind the stoyline, where a path that consists of a sequence of nouns and
verb frames. 

A single-hop classification can described as Equation~\ref{UHop_equation} and
Figure~\ref{fig:UHop}.
In step \(i\), at the current entity \(h_{i}\), the model is given a list of
candidate relations \(r_{i} \in R_{i}\) and entities \(t_{i} \in T_{i}\). Each
\(r_{i}\) is in [verb.\(t_{i}\)] or [verb.noun] format, containing both verb
frame and tail noun entity's information.
The scoring model \(F\) is given $objects$ and predicted relations
\(r_{1},...,r_{i-1}\) as input. The mode predicts a score for each \(r_{i}\)
and select the highest verb-noun pair \(r_{i}\) from \(Q\).

{
% \abovedisplayshortskip=-2pt 
% \belowdisplayshortskip=-7pt
\begin{small}
\begin{equation} 
    \label{UHop_equation}
    r_{i} = \mathop{\arg\max}_{q \in Q}  F(objects, r_{1},...,r_{i-1}).
\end{equation}
\end{small}
}
\paragraph{Training} UHop learns to pathfind a stoyline from the golden
storyline. The training procedure starts with an initial noun token entity
\texttt{$<$s0$>$} in golden storyline to perform a single hop classification,
where \(h_{1}=\) \texttt{$<$s0$>$}. It learn to select the correct relation
\(r_{i}\) from a list of candidate relations \(R_{i}\) in
\(\mathcal{G}_{\mathit{vg}}\) and \(\mathcal{G}_{\mathit{vist}}\). Then, it
calculates the error to noun and verb frame in the golden storyline for
back-propagation. In the next hop, the framework proceeds to the next noun in
golden storyline and repeats the single-hop classification.

\paragraph{Testing} 
% \subsection {Story Graph Construction} 
%To transform five images to a story graph, the system extracts story elements from the given five images.
In \system's testing step, for each story, fives images are transformed into a
story graph \(\mathcal{G}_{\mathit{story}}\). 
As demonstrated in Figure~\ref{fig:flowchart}, we first extract story elements
\(objects\) and \(terms\) for each stories. The story elements are linked
altogether using the verb frames in \(\mathcal{G}_{vist}\) and
\(\mathcal{G}_{vg}\) as edges. As a result, a
well-defined graph presenting a
comprehensive view of five images is created for each
story---\(\mathcal{G}_{\mathit{story}}\). Next, a trained UHop finds a
storyline in  \(\mathcal{G}_{\mathit{story}}\), where all entities are only the
\(objects\) and \(terms\) from the given five images. The framework starts with
\texttt{$<$s0$>$} to perform single hop classification, where \(h_{1}=\)
\texttt{$<$s0$>$}. Unlike training, it only selects \(r_{i}\) from \(R_{i}\)
listed in \(\mathcal{G}_{\mathit{story}}\). In the next hop, 
the previous predicted entities are used as start entity, \(h_{1}=t_{i-1}\). It
continues to hop from entity to entity until it reaches the next token
\texttt{$<$s1$>$}. The path from \texttt{$<$s{\scriptsize{i-1}}$>$} to
\texttt{$<$s{\scriptsize{i}}$>$} is called an event $e_{i}$. The path search
from \texttt{$<$s{\scriptsize{i}}$>$} to the next token
\texttt{$<$s{\scriptsize{i+1}}$>$} continues until the search is terminated by
termination decision described in UHop. Eventually, the model finds a storyline
of arbitrary length $L$, that is, a storyline contains any number of events:
$e_{1},...,e_{L}$.%, as demonstrated in  Figure~\ref{fig:flowchart}. 
% a non-exhaustive relation
% extraction framework to avoid high computation cost in path search.
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth]{figures/Uhop.pdf}
	 \caption{Storyline pathfinding process. A single-hop classification begins
	 with \texttt{dog}. The storyline predictor is given three candidates
	 relations; each in [verb.noun] format. The framework selects highest score
	 relation and move on to the next entity \texttt{park}. Then, the single-hop
	 classification repeats again. 
    % \yun{more detail?(a. input, b. navigate)}
    } 
    \label{fig:UHop}
\end{figure} 

\subsection{Framework Explanation}
%$(self\_motion)$ and $(self\_motion)$ express the same semantic meanings, but they represent different semantic meaning when including the tail entities such as  and . %In addition, including tail entities benefits entities association, such that, the models learns to select $(self\_motion, park)$ over $(self\_motion, sky)$. 
%\ethan{refer to Question 11} %Lastly, the tail entity decides the story flow for the rest of the storyplot as it'll become next hop's head entity.

%\ethan{do we need to explain how UHop work?}


%UHop selects entities hop by hop. 
%In each hop, UHop is given previous selected entities, relations and image features, as well as, a list of candidate entities and candidate relations. Based on the previous selections, UHop selects an appropriate entities from the candidate entities based the corresponding relations.

%Not only it learns what to go, it also learns where to go. 
%To optimize the relation prediction model, hinge loss is used and is defined as 
%\begin{equation} 
%    \mathcal{L} =\frac {\sum\limits_{r\in R-\hat{r}}\max(0, -(s^{\hat{r}} - s^r) + M)}{|R-\hat{r}|},
%\end{equation}
%On \(n^{th}\) hop, a HR-BiLSTM ~\cite{Yu_2018} was given a list of candidate relations \(R\) linked to current entities. To predict the next relation, the model used image objects and previous predicted relations and entities as inputs. 
HR-BiLSTM~\cite{Yu_2018} is adopted as the scoring model $F$. In $F$, 
$objects$ are converted to word embeddings via
GloVe~\cite{pennington2014glove} as {$E(object)$}. 
%The relations are composed by three elements: semantic frame, end entity, and image position. 
All relation embedding $\mathit{E}(r)$, 
%Previous predicted tuples and candidate tuples representation 
are decomposed into graphical embedding $\mathit{E}_{graph}$ and textual
embedding $\mathit{E}_{text}$. 
$\mathit{E}_{graph}$ transforms a verb frame $v$
and a tail entity's image position $p^{t}$ into a one-hot vector, denoting the
graphical and image positional information. 
%~\ethan{refer to Question 13} % which it applied to an arbitrary embedding layer, as they are input to an embedding layer to form a graphical embedding. 
$\mathit{E}_{text}$ is composed by the verb frame and tail entity word embedding.
Then, the $\mathit{E}_{graph}$ and $\mathit{E}_{text}$ are concatenated into one
representation $\mathit{E}(r)$. 
We formulate the representation of relation $r$ as

{
% \abovedisplayshortskip=-5pt 
% \belowdisplayshortskip=-7pt
\begin{small}
\begin{equation}
    \begin{split}
    \mathit{E}_{graph}(r) = [\mathbbm{1}(v) ; \mathbbm{1}(p^{t})], \\
    \mathit{E}_{text}(r) = [E_{w}(f); E_{w}(t)], \\
    \mathit{E}(r) = [\mathit{E}_{graph}(r) ; \mathit{E}_{text}(r)],
    \end{split}
\end{equation}
\end{small}
}
where $\mathbbm{1}(\cdot)$ returns the one-hot representation, and
$E_{w}(\cdot)$ returns the word embeddings via
GloVE, and [;] denotes concatenation.

A verb frame and tail entity are combined into $r_{i}$ due to relational
ambiguity issues among candidate relations.
%Although 
%UHop used previous predicted relation to predict the next relation. However, relation itself doesn't provide sufficient information. 
Using Figure~\ref{fig:UHop} as an example, given a head entity \emph{dog}, candidates
\emph{self\_motion.park} and \emph{self\_motion.owner} represent different semantic
meanings when tail entities \emph{park} and \emph{owner} are included. However,
excluding tail entities results in identical relation candidates
\emph{self\_motion} and thus the ambiguity between two different candidates.

%As the prediction model, HR-BiLSTM, iteratively predicts tuples, a termination
%decision is executed to terminate single-hop prediction, allowing the model
%to stop at the optimal hop length.
%at the same time. A UHop termination decision allows the model terminate the single hop prediction that gives us an optimal amount of hops. 
%After finishing storyline prediction, the predicted tuples are
%accumulated into a storyline. Finally, the framework uses $<$s$>$ to separate a
%storyline to a set of events $e_{1}...e_{L}$, as demonstrated in 
%Figure~\ref{fig:flowchart}. 
% \yun{How is the starting entity chosen?}
%according to training data's story length. %After generating a  complete storyplots, we divided a storyplots by using token $<s>$ and formed \ethan{termset??}. %\ethan{ termset??} will be used to generate $n$ sentences in stage 3. 

%\ethan{
%Questions:
% 9. feel free to edit the name: current candidate name: Storyline prediction, generation, extraction, development, composition. 

%10. We decided not to include penalty, it seems a bit minor, plus, we'll have a lot of analysis in the later pages. 

%11. is the reasoning/example too long?

%12. Do we need a diagram to explain hop relation extraction. 

%13. Can i call graphical representation? 
%Notes: 
%Add a flowchart of storyline plotting
%}

%In each hop, UHop would predict a relation from  % and equip an automatic termination mechanism.

%Each subgraph consisted abundant elements that represent image, we distilled and organized these elements to plot a storyline. 


\section{Stage 2: Story-Reworking}
In story reworking, the framework consists of two components: the story
generator and the story evaluator. The story generator generates a story
according to the storyline; the story evaluator--- a discriminator trained on
MTurk Human Ranking data to classify good and bad story--- outputs a story
quality score and modifies the loss functions.
%The story generator and story evaluator are inseparably interconnected, where
%the story generator reworks the story according to the story evaluation score, which
%reflects the quality of the generated story. %The story
%reworking stage revises and rewrites the drafts repeatedly, until optimal
%loss is reached. 
%Once a story is generated, the human judgement would rate a story and return a score. Then, the story generator edit its writing style accordingly to the scores, and return the story for human 

% In stage 2, a story generation model generates stories from storylines. Our story generation model consists two unique qualities: flexible input design and human-like story rating system. 

% -learn to write a story considering sentence-level and story-level

% -learn to edit stories by human-judgement.
\subsection{Story Generator} %A recurrent 
A storyline consists of a set of events  $e_{1}...e_{L}$, is inputted to the
story generator. The generator, a Transformer-based
~\cite{vaswani2017attention} framework, generates the story. 
%While most previous work overfits to 5 sentences stories in VIST dataset, 
Unlike most VIST models, the story generator is dynamic: the number of output
sentences is depending on the numbers of the events. 
To manage diverse number of events, the Transformer is designed as a sentence
generator which iteratively generates one sentence per event until it generates
$L$ sentences. 
%The story generator handles a variety of input length. 
%We proposed a Recurrent Transformer architecture to generates sentence iteratively which the amount of iterations is dependent to amount of events.
%. In other words, the amount of iterations is dependent on event's length. 
%according to input length. 
For each step $i$, event $e_{i}$ and the previous
predicted sentence $y_{i-1}
$%, and a memory embedding $m$ are input to the
%Transformer.  A memory layer is constructed using a conventional LSTM layer, which
%is given previous sentences $y_{1},...,y_{i-1}$ to accumulate historical knowledge
%and output a memory embedding,
%after which the Transformer predicts the next sentence $y_{i}$. 
are used to predict next sentence $y_{i}$.
After $L$ steps, the story generator outputs a story $s = y_{1},...y_{L}.$
%\subsubsection{Memory Embedding}

%\subsubsection{Hierarchical Story Generation} 

%At time step $i$, generating sentence $s_i$, the model receives a sentence level loss. As this model predicts one sentence at a time, the model is trained more efficient by back-propagating every sentence. Nevertheless, a story level loss is also consider to examine model's story level's performance. A story level loss is calculated after generating the entire story. \yun{can move MLE loss description here}

% \begin{equation} 
%     \mathcal{L}_{sen}(\theta) = - \sum_{\ell=1}^{L} log(p_{\theta}(y_{\ell}| e_{\ell}, m_{\ell},  y_{1}, ..., y_{\ell-1})),
% \end{equation}
% \begin{equation} 
%     \mathcal{L}_{story}(\theta) = - log(p_{\theta}(s|e_{1:L}, y_{1},..., y_{L})),
% \end{equation}
% story level loss to complement such disadvantage. 

\subsection{Story Evaluator}
%After writing a preliminary story, human writers repetitively edit their stories to improve story quality. 
%If we have a dataset that asks human to score the generated stories, it is more possible for model to generate more human-like stories.
%However, it is unlikely to collect all the generated stories in VIST task, and asking human to label the stories is time consuming and expensive.
%By using human evaluation data from ~\cite{hsu2020knowledge}
Most previous VIST works use human evaluations to examine the quality of their
work by crowdsourcing, comparing their generated stories with baselines'
stories. In this paper, we use first and last place stories in MTurk Human
Ranking data as positive and negative samples. The story-evaluator, a
discriminator trained on MTurk Human Ranking data, learns to distinguish
positive and negative samples. It outputs a score for each story, and the
scores are converted into rewards, as shown below:
%We attempt to use the result of human evaluation and design a reward function to mimic human judgement. 

% the KG-Story~\cite{hsu2020knowledge} 
% results from AMT.
% This data contains two experiments, samples of 1,000 stories generated by all
% the baselines for the same photo sequence.
% Specifically, AMT workers were asked to rank AREL~\cite{wang2018show},
% human-written ground-truth stories, using 3 different settings of their model in
% each experiment.
% We separate stories ranked 1 and 5 into positive and negative samples,
% respectively. 
%As this ranking data contains the comparison with human-written stories, it provide the global view of the story quality.
%The model is first given the sequence representation of story $s$, after which we
%apply a linear layer to the sequence representation followed by a $\mathrm{tanh}$
%function and a softmax function to predict a binary label\yun{can delete, can tell from eq3 and 4}.
{
% \abovedisplayshortskip=-15pt 
% \belowdisplayshortskip=-10pt
\begin{small}
\begin{equation} 
    p_{\mathit{LM}}(u|s) = {\rm softmax}({\rm tanh}(\textbf{W} \mathit{LM}(s)) + \textbf{b} ),
\label{scoring_stories}
\end{equation}
\end{small}
}
{
% \abovedisplayshortskip=-15pt 
% \belowdisplayshortskip=5pt
\begin{small}
\begin{equation} 
    \mathcal{R}(s) = - p_{\mathit{LM}}(u|s) + c
\label{reward_scoring}
\end{equation}
\end{small}
}
$\mathit{LM}(\cdot)$ is a GRU language model ~\cite{cho2014learning}; $u=1$
indicates story $s$ is a positive sample and $u=0$ indicates $s$ is a negative
sample. $p_{\mathit{LM}}(\cdot)$ returns a score from 0 to 1 to reflect story
quality. 
%When generating stories, we use lower loss for more positive stories.
The story-evaluator $\mathcal{R}(\cdot)$ returns a reward, an inverse of
$p_{\mathit{LM}}(\cdot)$ with coefficient $c$ = 1.5. The reward later
manipulates the loss, optimizing toward human preference. Note the story
evaluator was pre-trained in advance. 
%\yun{need to change description}

%During training phase, we replace Equation \ref{story_equation} to Equation \ref{reward_equation} in order to revise the story.
%After returning a score from story evaluator, story generator back-propagate with the  %then revises the preliminary story $s =
%y_{1}', ..., y_{L}'$ to the refined story $s = y_{1}'', ...,
%y_{L}''$. 
% After story evaluator calculating the score%human-judgment reward function
% , the preliminary story $s =
% y'_{1}, ..., y'_{L}$ is transferred to the refined story $s' = y''_{1}, ...,
% y''_{L}$.

\subsection{Optimization with Story Evaluator}
For optimization, the story generator receives two types of loss functions:
sentence-level and story-level.
%Maximum likelihood estimation (MLE) finds an optimal solution for the story generation model.
Given reference $y^*_{1},...,y^*_{L}$ and predicted story $y_{1},...,y_{L}$, in
our Maximum Likelihood Estimation (MLE) optimization process, in each step from
1 to $L$, the model predicts a sentence $y_{i}$ to calculate the loss between
$y_{i}$ and $y^*_{i}$ and back-propagates, as shown in Figure~\ref{fig:loss}.
%over current event and previous sentences.
%After the generation model finishes predicting
After predicted $L$ sentences, in story-level optimization, the model predicts
$y_{1},...,y_{L}$ to calculate negative log-likelihood to the reference
$y^*_{1},...,y^*_{L}$ and back-propagates. 
The sentence-level and story-level optimization by MLE on data
$\mathcal{D}$ are formulated as 

{
% \abovedisplayshortskip=-3pt 
% \belowdisplayshortskip=-15pt
\begin{small}
\begin{equation} 
\label{sen_equation}
    J^{\mathit{MLE}}_{\mathit{sen}}(\theta, \mathcal{D}) = 
    \sum_{Y \in \mathcal{D}} - \log p_{\theta}(y_{i}| e_{i}, y_{i-1}), 
\end{equation}
\end{small}
}
{
% \abovedisplayshortskip=-15pt 
% \belowdisplayshortskip=-30pt
\begin{small}
\begin{equation} 
\label{story_equation}
    J^{\mathit{MLE}}_{\mathit{story}}(\theta, \mathcal{D}) = 
    \sum_{Y \in \mathcal{D}} \frac{1}{L}\sum_{i=1}^{L} - \log p_{\theta}(y_{i}'| e_{i}, y_{i-1}'),
\end{equation}
\end{small}
}
where $e_{i}$%, $m_{\ell}$
, and $y_{i}$ denote the $i$-th event, %the memory embedding,  
and the sentence respectively. 
%, noting that $m_{\ell}$ is the hidden
%state output of LSTM by inputting $y_1$ to $y_{\ell-1}$.
$y_{i}'$ represents the updated sentence after sentence level optimization. %and $e_{1:L}$ denotes all $L$ events in the storyline.
$\theta$ represents the parameter of story generation model and is updated
using Adam~\cite{kingma2014adam}. 

After training for 30 epochs, story-evaluater begins to manipulate the
story-level loss. Inspired by Reinforcement Learning~\cite{10.1007/BF00992696},
which utilizes reward to guide the training process, we use the story evaluator
$\mathcal{R}(\cdot)$ to encourage the generation model to focus on stories
preferred by humans.
The reward is directly multiply to story-level loss as shown below:

% \begin{equation} 
%     \mathcal{L}_{story(reward)}(\theta) = \mathcal{R}(s) \mathcal{L}_{story}(\theta).
% \end{equation}
{
% \abovedisplayshortskip=-30pt 
% \belowdisplayshortskip=-30pt
\begin{small}
\begin{equation} 
    \label{reward_equation}
    % J^{\mathit{reward}}_{\mathit{story}}(\theta, \mathcal{D}, s) = 
    % \sum_{Y \in \mathcal{D}} \frac{\mathcal{R}(s)}{L}\sum_{i=1}^{L} - \log p_{\theta}(y_{i}'| e_{i}, %m_{\ell}, 
    % y_{i-1}'),
    J^{\mathit{reward}}_{\mathit{story}}(\theta, \mathcal{D}) = 
    \begin{cases}
    J^{\mathit{MLE}}_{\mathit{story}} & \text{if epoch $\leq$ 30}\\
    \mathcal{R}(s)J^{\mathit{MLE}}_{\mathit{story}} & \text{if 30 $<$ epoch $\leq$ 60}
    \end{cases}
\end{equation}
\end{small}
}
% where $y'_{i}$ is the updated sentence after sentence-level optimization and $\theta$ is the stochastic
% gradient descent for model parameter. %Training for 60 epochs, the story generator is back-propagated by the Equation~\ref{story_equation} for 30 epochs. After 30 epochs, the story generator is back-propagated by the Equation~\ref{reward_equation}, where the story generator is optimized with human preference loss. \yun{revision needed for the equation}
% \input{tables/algorithm}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.95\linewidth ]{figures/loss.pdf}
	 \caption{Optimization flowchart for story generator. For step 1 to $L$, the
	 model is optimized by sentence level loss. In step $L+1$, all sentences are
	 generated, and the model is optimized by the reward story loss.}
    \label{fig:loss}
\end{figure}


==> origin/relatedwork-orig.tex <==
\section{Related Work} 

Visual storytelling (VIST) was proposed by~\citet{huang2016visual}.
%Researchers have been exploring ways to improve VIST models primarily in two directions:
So far, there are two lines of research tackling different aspects of this
task.
One strand focuses on developing models or adopting various training techniques
on the VIST dataset only.
Some modify end-to-end recurrent model architectures for better story
generation~\cite{hsu2018using,gonzalez2018contextualize,kim2018glac,huang2019hierarchically,
Jung2020HideandTellLT}, and others use adversarial training to generate
more diverse
stories~\citep{chen2017multimodal,wang2018show,DBLP:journals/corr/abs-1804-09160,
hu2019makes}.
%However, the methods in this category often overfit on the knowledge and the vocabulary of VIST training data.
However, these methods still generate caption-like stories, which remain
monotonous and repetitive.
% \yun{without KG: model structure or learning method}

The other strand focuses on leveraging external sources to enrich story
contents. Current studies on knowledge graph and language model integration
have shown to be beneficial~\citep{
% lobue-yates-2011-types,
bowman-etal-2015-large,  hayashi2019latent, zhang-etal-2017-ordinal,
ijcai2018-643,
yang-etal-2019-enhancing-topic}.
In recent VIST studies, \citet{pengchengKnowledge2019} apply ConceptNet~\citep{liu2004conceptnet}
and self-attention for common-sense augmented image features.
\citet{Wang2020StorytellingFA} use
graph convolution networks~\cite{DBLP:journals/corr/abs-1804-01622} on scene
graphs to associate objects across images.
%Both of graph-based approaches encoded knowledge graph into feature space, following by an end-to-end model architecture. \ethan{it's contradicting}
%However, most end-to-end models overfit to the knowledge and the story length of VIST training data. The stories are restricted to five sentence, which the story contents are relatively limited. \yun{align intro} \ethan{pls refer to Question 7.}
KG-Story~\cite{hsu2020knowledge} is a three stage framework to cohere
story contents, which uses the Visual Genome knowledge graph~\cite{Krishna_2017}
to add semantic relations between two adjacent images. 
%Although implementing knowledge graph, these methods cannot cohere the visual elements' relation for five images.
%Moreover, the sentence of these stories cannot consider more than one image's information.\yun{need stronger disadvantage for KG-based methods?}
In addition, current automatic storytelling studies have demonstrated the
effectiveness of story plotting~\cite{DBLP:journals/corr/abs-1811-05701,
DBLP:journals/corr/abs-1902-01109}, which typically involves organizing the
ingredients into a well-organized sequence of events. Nevertheless, none of the
studies have considered story plotting in visual storytelling. 
In this paper, we challenge current leading models by fully utilizing story
plotting and knowledge graphs, achieving greater image and story coherence. 
%The story plotting was used to organize the entities from a comprehensive perspective. Being able to view the entire image stream, the model is capable of associating inner-inter relations and arranging visual elements across-with images. 
% \ethan{may add some advantages of knowledge graph}


%However, none of the visual storytelling studies have considered story plotting before story generation, which storyplotting arranges the visual elements and organizes the story flow before writing a story. %Plotting a storyline is essential and has shown beneficial for storytelling task 
% ~\ethan{pls refer to Qeustion 8}
%Therefore, we introduced storyplotting to VIST, aim to organize the visual elements and enrich story contents. 
%Unlike caption-like visual stories, the predicted storyline models appropriate relation between visual elements within and across the images and flexibly generate cohesive stories based on this storyline.\yun{need to be edited}

% \yun{with KG: encode kg or find relation(KG-Story)}
% didn't fully utilize KG and can only tell a story with uni-direction
% appropriate relation that connects 5 images
% Non of the above work considers plotting storyline that organizes the visual and textual elements

Several works show that language generation models often result in
problematic grammar or favor generic 
utterances~\cite{DBLP:journals/corr/LiGBGD15, DBLP:journals/corr/ShaoGBGSK17}.
Therefore, there is a growing interest in developing an editing model beyond
the generation model~\cite{bahdanau2014neural, dblp:journals/corr/abs-1709-08878}.
Editing models have also been applied to several vision-to-language 
tasks~\cite{kuznetsova-etal-2013-generalizing, 10.5555/2566972.2566993}, and
\citet{DBLP:journals/corr/abs-1906-01764} consider editing within VIST, 
proposing VIST-Edit.
Arguing that machine-generated stories are still far from human, VIST-Edit
trains another generation model and rewrites machine-generated stories.
% Applying editing to VIST, \citeauthor{DBLP:journals/corr/abs-1906-01764} first introduced Post-Editing, claiming the machine generated stories are still far from human.
% By training another generation model, the model rewrites machine generated stories from prior works. 
Other VIST studies adopt editing in their model design.
For example, modifying the model architecture to alter the writing style, \citet{hu2019makes}
propose a reward function with three aspects, and
\citet{10.1145/3323873.3325050} customize the emotion for the generated stories.
Since most methods optimize their stories on automatic metrics, their
algorithms do not necessarily align to human standards.  
Therefore, we present a novel rating approach that refines stories by leveraging
the human evaluation data of prior studies, which consists of human annotated scores 
for each generated story.

%\ethan{
%Questions:

%7. UHop does have the ability to manipulate the length of the storyline, but should we even mention diverse length in this paper, since the focus is plotting and editing? If yes, should we edit the introduction to include this advantage?

%8. not sure if the reasoning is strong enough (reason for using story plotting)
%}


==> origin/result-orig.tex <==
\subsection{Evaluation Results}

\input{human-eval-result.tex}

\paragraph{Automatic Evaluations}
\input{auto-eval-result}





==> tables/ablation.tex <==
\begin{table}
\begin{center}
\small
\scalebox{0.84}{

\begin{tabular}{lccc}
\hline
  & {\system} & {\system} w/o R & {\system} w/o PR\\
\hline
Avg rank & 1.95 (0.79) & 2.00 (0.80) & 2.03 (0.85)\\
Majority rank & 1.93 & 2.02 & 2.08\\
\hline
\end{tabular}}
\end{center}
\caption{Ablation study result of proposed method in two configurations,
without reworking (w/o R) and without plotting and reworking (w/o PR). Numbers in brackets
indicate standard deviation of stories' rank. \yun{ablation study examples?}
}
\label{tb:ablation}
\end{table}


==> tables/ablation_test-orig.tex <==
\begin{table}
\begin{center}
\small
\scalebox{0.8}{

\begin{tabular}{lcccccccc}
\hline
  & $objects$ & $terms$ & \(\mathcal{G}_{\mathit{vg}}\) & \(\mathcal{G}_{\mathit{vist}}\) & Plot & Rework & Avg & Major\\
\hline\hline
&
\checkmark & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & 1.89 & 1.87\\
1&
 & \checkmark & \checkmark & \checkmark &  \checkmark & \checkmark  & 1.98 & 2.00\\
 &
\checkmark &  & \checkmark & \checkmark & \checkmark  &  \checkmark & 2.12 & 2.13\\
\hline
&
\checkmark & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & 1.97 & 1.94\\
2&
\checkmark & \checkmark &  & \checkmark &  \checkmark & \checkmark  &1.98 & 1.99\\
&
\checkmark & \checkmark & \checkmark &  & \checkmark  &  \checkmark & 2.00 & 2.06\\
\hline

&
\checkmark & \checkmark & \checkmark & \checkmark &  \checkmark &  \checkmark & 1.95 & 1.93\\
3 &
\checkmark & \checkmark & \checkmark & \checkmark &  \checkmark &  & 2.00 & 2.02\\
&
\checkmark & \checkmark & \checkmark & \checkmark &   &   & 2.03& 2.08\\

\hline

\end{tabular}}
\end{center}
\caption{Human evaluation results for ablation studies: 1. Story elements 2.
Knowledge Graph 3. Plot and Rework. {\system} outperforms in all ablation
settings, indicating the importance of using all components.}
\label{tb:ablation_test}
\end{table}


==> tables/algorithm.tex <==
\begin{algorithm}[t]
  \caption{Story Reworking}
  \begin{algorithmic}[1]

  \For{ episode $\gets 1$ to $N$ }
    \For{ length $\gets 1$ to $L$ }
      \State $\theta \gets \theta + \eta \frac{\partial \mathcal{J}^{\mathit{MLE}}_{\mathit{sen}}(\theta, \mathcal{D})}{\partial \theta}$ (see Eq.~\ref{sen_equation})
    \EndFor 
    \State collect preliminary story $s$ = $y_{1}', ..., y_{L}'$ 
    
    %$\theta \gets \theta + \eta \frac{\partial \mathcal{J}^{\mathit{MLE}}_{\mathit{story}}(\theta, \mathcal{D})}{\partial \theta}$  (see Eq.~\ref{story_equation})\\
    %generate story $s$ = $y_{1}, ..., y_{L}$
    
    %\If{Using Reward}
    \State$\theta \gets \theta + \eta \frac{\partial \mathcal{J}^{\mathit{reward}}_{\mathit{story}}(\theta, \mathcal{D}, s)}{\partial \theta}$ (see Eq.~\ref{reward_equation})
    %\EndIf
    
    \State collect refined story $s$ = $y_{1}'', ..., y_{L}''$
    \EndFor
    \label{code:generation}
  \end{algorithmic}
\end{algorithm}


==> tables/automatic.tex <==
\begin{table*}
\begin{center}
\small
\scalebox{1}{
% \begin{tabular}{lcccccccccccc}
% \hline
%  Methods & M & R & C & B-4 & MLTD & voc-d & \(r_{e}\)-4 & \(r_{e}\)-5 & \(R_{bert}\) & \(P_{bert}\) & \(F_{bert}\) & BLEURT\\
% \hline\hline
% AREL  & 35.4 & 30.5 & 9.36 & 14.4 & 22.45 & 0.53 & 94.31\% & 92.03\% & 0.845 & 0.869 & 0.857 & 51.55 \\
% GLAC  & 33.7 & 27.3 & 4.94 & 10.7 & 32.87 & 0.67 & 90.71\% & 87.43\% & 0.844 & 0.872 & 0.858 & 71.22\\
% % ReCo-RL \cite{hu20aaai} & 35.8 & 29.5 & 11.9 & 13.5 \\
% KG-Story  & 32.2 & 27.2 & 7.96 & 9.93 & 40.52 & 0.71 & 81.07\% & 76.71\% & 0.847 & 0.862 & 0.854 & 71.94 \\

\begin{tabular}{lccccccccc}
\hline
 Methods & M & R & C & B-4 & BLEURT & MLTD & voc-d & \(r_{e}\)-4 & \(r_{e}\)-5 \\
\hline\hline
AREL  & 35.4 & 30.5 & 9.36 & 14.4 & 0.515 & 22.45 & 0.53 & 94.31\% & 92.03\%  \\
GLAC  & 33.7 & 27.3 & 4.94 & 10.7 & 0.712 & 32.87 & 0.67 & 90.71\% & 87.43\% \\
% ReCo-RL \cite{hu20aaai} & 35.8 & 29.5 & 11.9 & 13.5 \\
KG-Story  & 32.2 & 27.2 & 7.96 & 9.93 & 0.719 & 40.52 & 0.71 & 81.07\% & 76.71\%  \\
{\system}  & 31.6 & 26.4 & 8.7 & 7.65 &  & 45.79 & 0.73 & 75.81\% & 71.05\%\\
% \hline 
% \textbf{Our Baselines} &  & & & \\

% \hline
% Ours w/o something &  & & & \\
% Ours w/o something &  & & & \\
% \hline
% Ours  &  & & & & & & & \\
\hline
\end{tabular}}
\end{center}
\caption{Automatic evaluation results for generated stories by models and baselines. M, R, C, and B-4 denote METEOR, ROUGE-L, CIDEr, and 4-gram precision score of BLEU metric, respectively. MTLD and voc-d are two settings of lexical diversity. 
% \(r_{e}\)-4 and \(r_{e}\)-5 represent 4- and 5-gram inter-story repetition.
% The recall, precision, and F1 scores from BERTScore annotate as \(R_{bert}\), \(P_{bert}\), and \(F_{bert}\), respectively.
}
\label{tb:auto_eval}
\end{table*}

% \begin{table*}[]
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \multirow{Methods} & \multicolumn{2}{c|}{lexical diversity} & \multicolumn{2}{c|}{inter-story repetition} & \multicolumn{3}{c|}{BERTScore} & \multirow{BLEURT} \\ \cline{2-8}
%  & MTLD & voc-d & 4-gram & 5-gram & R & P & F & \\ \hline
% AREL & & & & & & & & \\
% GLAC & & & & & & & & \\
% KG-Story & & & & & & & & \\
% OURS & & & & & & & &
% \end{tabular}
% \end{table*}

==> tables/automatic_diverse.tex <==
\begin{table}
\begin{center}
\small
\scalebox{1}{


\begin{tabular}{lccccc}
\hline
Method & MLTD & voc-d & \(r_{e}\)-4 & \(r_{e}\)-5 & \# Sent \\
\hline\hline
AREL  & 22.45 & 0.53 & 94.31\% & 92.03\% & 5.0 \\
GLAC  & 32.87 & 0.67 & 90.71\% & 87.43\% & 5.0\\
KG-Story  & 40.52 & 0.71 & 81.07\% & 76.71\% & 5.81  \\
{\system}  &  \textbf{45.79} &  \textbf{0.73} &  \textbf{75.81\%} &  \textbf{71.05\%} &  \textbf{5.96}\\



\hline
\end{tabular}}
\end{center}
\caption{Lexical diversity (i.e., MLTD and voc-d), 4- and 5-gram inter-story
repetition rate (i.e., $r_{e}$), and the average number of sentences
}
\label{tb:auto_diverse}
\end{table}


==> tables/automatic_gram.tex <==
\begin{table}
\begin{center}
\small
\scalebox{0.87}{

\begin{tabular}{lccccc}
\hline
Method & METEOR & ROUGE-L & CIDEr & BLEU-4 & BLEURT \\
\hline\hline
AREL  & \textbf{35.4} & \textbf{30.5} & \textbf{9.36} & \textbf{14.4} & 0.515 \\
GLAC  & 33.7 & 27.3 & 4.94 & 10.7 & 0.712 \\
KG-Story  & 32.2 & 27.2 & 7.96 & 9.93 & 0.719 \\
{\system}  & 31.6 & 26.4 & 8.70 & 7.65 & \textbf{1.372} \\
\hline
\end{tabular}}
\end{center}
\caption{Automatic evaluation results for generated stories on n-gram based
metrics and BERT-based metric (BLEURT)\yun{delete some metrics without misunderstanding}}
\label{tb:auto_gram}
\end{table}


==> tables/baseline_rank-orig.tex <==
\begin{table}
\begin{center}
\small
\scalebox{0.82}{

\begin{tabular}{lcccccc}
\hline
Method & 1st & 2nd & 3rd & 4th & Avg & Major \\
\hline\hline
AREL  & 20.6\%(258) & 26.8\% & 27.2\% & 25.4\% & 2.57 & 2.56 \\
GLAC  & 21.7\%(271) & 24.2\% & 25.5\% & 28.6\% & 2.61 & 2.73\\
KG-Story  & 25.1\%(314) & 25.2\% & 25.7\% & 24.0\% & 2.49 & 2.53  \\
{\system}  & \textbf{32.6\%}(\textbf{407}) & 23.7\% & 21.7\% & \textbf{22.0\%} & \textbf{2.33} & \textbf{2.28}\\
\hline

% \hline
% Method & 1st & 2nd & 3rd & 4th & Avg rank \\
% \hline\hline
% AREL  & 20.6\%(258) & 26.8\% & 27.2\% & 25.4\%(317) & 2.57 \\
% GLAC  & 21.7\%(271) & 24.2\% & 25.5\% & 28.6\%(357) & 2.61\\
% KG-Story  & 25.1\%(314) & 25.2\% & 25.7\% & 24.0\%(300) & 2.49  \\
% {\system}  & \textbf{32.6\%}(\textbf{407}) & 23.7\% & 21.7\% & \textbf{22.0\%}(\textbf{276}) & \textbf{2.33} \\
% \hline

% \hline
% Method & AREL & GLAC & KG-Story & {\system} \\
% \hline\hline
% 1st & 20.6\%(258) & 21.7\%(335) & 25.1\%(340) & 32.6\%(317) \\
% 2nd & 26.8\% & 24.2\% & 25.2\% & 23.7\% \\
% 3rd & 27.2\% & 25.5\% & 25.7\% & 21.7\% \\
% 4th & 25.4\% & 28.6\% & 24.0\% & 22.0\% \\
% Avg rank & 2.57 & 2.61 & 2.49\% & \textbf{2.33} \\
% AREL  & 20.6\% & 26.8\% & 27.2\% & 25.4\% & 2.57 \\
% GLAC  & 21.7\% & 24.2\% & 25.5\% & 28.6\% & 2.61 \\
% KG-Story  & 25.1\% & 25.2\% & 25.7\% & 24.0\% & 2.49  \\
% {\system}  & 32.6\% & 23.7\% & 21.7\% & 22.0\% & \textbf{2.33} \\

\end{tabular}}
\end{center}
\caption{Human ranking evaluation between {\system} and three methods. First
four columns indicate percentage of workers' ranking for each method, and the
fifth and the last column denote average and majority rank (1 to 4, lower is
better). Numbers in brackets indicates the quantity of the best stories for
each method. {\system} is significantly better than all baselines with
$\rho < 0.05$.} 
\label{tb:human_ranking}
\end{table}


==> tables/new_auto-orig.tex <==
% \begin{table*}
% \begin{center}
% \small
% \scalebox{1}{

% \begin{tabular}{lcccccccc}
% \hline
% Method & BLEU-4 & METEOR & BLEURT & MLTD & voc-d & \(r_{e}\)-4 & \(r_{e}\)-5 & \# Sent\\
% \hline\hline
% AREL  & \textbf{14.4} & \textbf{35.4} & 0.515 & 22.45 & 0.53 & 94.31\% & 92.03\% & 5.0 \\
% GLAC  & 10.7 & 33.7 & 0.712 & 32.87 & 0.67 & 90.71\% & 87.43\% & 5.0 \\
% KG-Story  & 9.93 & 32.2 & 0.719 & 40.52 & 0.71 & 81.07\% & 76.71\% & 5.81  \\
% {\system}  & 7.65 & 31.6 & \textbf{1.372} &  \textbf{45.79} &  \textbf{0.73} &  \textbf{75.81\%} &  \textbf{71.05\%} &  \textbf{5.96} \\
% \hline
% \end{tabular}}
% \end{center}
% \caption{}
% \label{tb:auto_new}
% \end{table*}

\begin{table}
\begin{center}
\small
\scalebox{0.84}{
\begin{tabular}{lccccc}
\hline
Method & BLEU-4 & METEOR & BLEURT & MLTD & voc-d\\
\hline\hline
AREL & \textbf{14.4} & \textbf{35.4} & 0.52 &  22.45  & 0.53\\
% \hline
GLAC & 10.7 & 33.7 & 0.71 &  32.87    & 0.67  \\
% \hline
KG-Story & 9.93 & 32.2 & 0.72  & 40.52   & 0.71\\
% \hline
{\system} & 7.65 & 31.6 & \textbf{1.37} &\textbf{45.79} &  \textbf{0.73}\\
\hline



% \multicolumn{6}{c}{(a) Reference-based evaluation results.} \\
% & &  &  \\
% \hline
% Method & \(r_{e}\)-4 & \(r_{e}\)-5 & \#  MLTD \\
% \hline\hline
% AREL   &  94.31\%    & 92.03\%     & 22.45 \\
% \hline
% GLAC   &  90.71\%    & 87.43\%     & 32.87 \\
% \hline
% KG-Story & 81.07\%   & 76.71\% & 40.52   \\
% \hline
% {\system} &\textbf{75.81\%} &  \textbf{71.05\%} &  \textbf{45.79}  \\
% \hline
% \multicolumn{4}{c}{(b) Lexical richness evaluation results.}
%\multicolumn{9}{c}{(a) Automatic evaluation results.} &  & \multicolumn{6}{c}{(b) Human evaluation results.}
\end{tabular}}
\end{center}
\caption{The first two columns show results of classic n-gram based metrics.
The third column shows BERT-based metric (BLEURT).
The last two columns show lexical diversity evaluation result(MLTD and voc-d).
% for generated stories. 
The high performance in lexical diversity metrics results low performance for
n-gram metrics. 
%Regardless of n-gram metrics, {\system} is significantly better than all baseline methods with $\rho < 0.05$.
}
\label{tb:auto_new}
\end{table}

% \begin{table*}
% \small
% \scalebox{0.76}{
% \begin{tabular}{lccccccccllccccc}
% \cline{1-9} \cline{11-16}
% Method & BLEU-4 & METEOR & BLEURT & MLTD & voc-d & \(r_{e}\)-4 & \(r_{e}\)-5 & \# Sent &  & Method & 1st & 2nd & 3rd & 4th & Avg rank\\
% \cline{1-9} \cline{11-16} 
% AREL & \textbf{14.4} & \textbf{35.4} & 0.515 & 22.45 & 0.53 & 94.31\% & 92.03\% & 5.0 &  & AREL &20.6\%(258) & 26.8\% & 27.2\% & 25.4\%(317) & 2.57\\
% GLAC & 10.7 & 33.7 & 0.712 & 32.87 & 0.67 & 90.71\% & 87.43\% & 5.0 &  & GLAC &21.7\%(271) & 24.2\% & 25.5\% & 28.6\%(357) & 2.61\\
% KG-Story & 9.93 & 32.2 & 0.719 & 40.52 & 0.71 & 81.07\% & 76.71\% & 5.81 &  & KG-Story &25.1\%(314) & 25.2\% & 25.7\% & 24.0\%(300) & 2.49\\
% {\system} & 7.65 & 31.6 & \textbf{1.372} &  \textbf{45.79} &  \textbf{0.73} &  \textbf{75.81\%} &  \textbf{71.05\%} &  \textbf{5.96} &  & {\system} &\textbf{32.6\%}(\textbf{407}) & 23.7\% & 21.7\% & \textbf{22.0\%}(\textbf{276}) & \textbf{2.33}\\
% \cline{1-9} \cline{11-16} 
% \multicolumn{9}{c}{(a) Automatic evaluation results.} &  & \multicolumn{6}{c}{(b) Human evaluation results.}
% \end{tabular}}
% \caption{(a)First three columns show the automatic evaluation results for generated stories on n-gram based metrics and BERT-based metric (BLEURT). Column 4-8 show the lexical diversity (i.e., MLTD and voc-d), 4- and 5-gram inter-story
% repetition rate (i.e., $r_{e}$), and the average number of sentences. (b) Human ranking evaluation between {\system} and three methods. 
% First four columns indicate percentage of workers' ranking for each
% method, and last column denotes average rank (1 to 4, lower is
% better). Numbers in brackets indicates the quantity of the best and the worst stories for each method.
% {\system} is significantly better than all baseline methods with
% $\rho < 0.05$.}
% \end{table*}

